Measuring Your ASTE Models in The Wild: A Diversified Multi-domain Dataset For Aspect Sentiment Triplet Extraction

Aspect Sentiment Triplet Extraction (ASTE) is widely used in various applications. However, existing ASTE datasets are limited in their ability to represent real-world scenarios, hindering the advancement of research in this area. In this paper, we introduce a new dataset, named DMASTE, which is manually annotated to better fit real-world scenarios by providing more diverse and realistic reviews for the task. The dataset includes various lengths, diverse expressions, more aspect types, and more domains than existing datasets. We conduct extensive experiments on DMASTE in multiple settings to evaluate previous ASTE approaches. Empirical results demonstrate that DMASTE is a more challenging ASTE dataset. Further analyses of in-domain and cross-domain settings provide promising directions for future research. Our code and dataset are available at https://github.com/NJUNLP/DMASTE.

==> chapters/0_abstract.tex <==
\begin{abstract}
Annotations for Aspect Sentiment Triplet Extraction (ASTE) are labor-intensive and time-consuming, resulting in lacking labeled data in many domains. 
% Prior works on Aspect Sentiment Triplet Extraction (ASTE) always rely on a large amount of labeled data, which is impractical for applications.
Therefore, we first propose to investigate ASTE in the cross-domain setting, which focuses on transferring knowledge from a resource-rich source domain to a resource-poor target domain. 
% However, existing ASTE datasets only cover two domains, and the reviews in these datasets are monotonous, which may limit the research.
% To advance cross-domain research in ASTE, we construct a new benchmark dataset Multi-Domain ASTE (\textbf{\datasetwb}). 
Due to limited domains and monotonous reviews, existing ASTE datasets may restrict the research in cross-domain ASTE. 
To promote related research, we manually annotate the Multi-domain ASTE (\textbf{\datasetwb}) dataset.  It covers four source and four target domains, providing more transfer pairs for cross-domain research. 
% 这句话放到这里显得上下不连贯
% Thus, \dataset enables sufficient correlation analysis between the model performance and domain discrepancy. 
Besides, the reviews in \dataset are of various lengths and expressed in assorted sentence patterns, which are more consistent with the real scenarios.
% Based on \datasetwb, we re-implement some representative methods in ASTE. Besides, we integrate some of them with the domain adversarial learning method, a common method in the cross-domain setting. 
% Furthermore, we conduct extensive empirical experiments in in-domain, single-source, and multi-source domain adaptation scenarios to investigate the challenges introduced by \datasetwb.
We conduct experiments on \dataset in multiple settings, analyze challenges introduced by \dataset in the domain adaptation setting, and provide promising directions for future research. 
% analyze results
\footnote{Our dataset and code will be available once accepted. }
\end{abstract}

==> chapters/1_intro.tex <==

\section{Introduction}
\label{sec:intro}

Aspect sentiment triplet extraction \citep[ASTE;][]{peng2020knowing} is a subtask in  aspect-based sentiment analysis (ABSA; \citealp{pontiki-etal-2014-semeval}). It aims to extract sentiment triplets from a given review, i.e., \textit{(aspect term, opinion term, sentiment polarity)}. As shown in Figure \ref{fig:intro-example}, one triplet in the example is (\textit{"curly cord"}, \textit{"hate"}, \textit{NEG}), which expresses \textit{negative} sentiment toward aspect term \textit{"curly cord"} with the opinion term \textit{"hate"}. 
% The second one is (\textit{"wire holders"}, \textit{"work"}, POS),  expressing \textit{positive} sentiment toward \textit{"wire holders"} with opinion term \textit{"work"}. 
\begin{figure}[htbp] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering
\includegraphics[width=0.45\textwidth]{figures/intro-example.pdf} 
\caption{An Example for the ASTE task. The terms highlighted in blue are aspect terms. The terms in orange are opinion terms. The words in green are sentiment polarities. "NULL" denotes the implicit aspect.} 
\label{fig:intro-example} %用于文内引用的标签
\end{figure}

Prior ASTE methods \citep{yan-etal-2021-unified, xu-etal-2021-learning} have achieved promising results through supervised learning  on a large amount of labeled data. 
However, annotating the ASTE data is labor-intensive and time-consuming for the following reasons:
(1) One instance can include multiple triplets. And there are three factors to be annotated for each triplet. (2) In each instance, one aspect can correspond to multiple opinions, and vice versa. (3) One instance can contain different sentiments. The complexity of annotating ASTE data leads to lacking labeled data in many domains.  
Therefore, we propose to explore the ASTE task in the cross-domain setting \citep{pan2009survey}, which aims to transfer knowledge from a resource-rich source domain to a resource-poor target domain. 


\begin{figure*}
     \centering
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figures/num_data.pdf}
    %      \caption{ }
    %      \label{fig:intro-num-data}
    %  \end{subfigure}
    %     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[trim=4 4 4 4,clip,width=\linewidth]{figures/length.pdf}
         \caption{Distribution of instance length.}
         \label{fig:intro-length}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[trim=4 4 4 4,clip,width=\linewidth]{figures/pos.pdf}
         \caption{Distribution of the number of POS 2-gram.}
         \label{fig:intro-pos}
     \end{subfigure}
        \caption{Comparisons between 14Lap and Electronics on instance length and the number of POS 2-grams per instance. The statistics of 14Lap and Electronics are from \citet{xu-etal-2020-position} and \datasetwb, respectively.
        }
        \label{fig:intro-cmp}
\end{figure*}


Although it is of great necessity to explore cross-domain ASTE,  the existing datasets for ASTE have the following deficiencies:
\begin{itemize}
    \item \textbf{Limited domains.} All existing ASTE datasets \citep{peng2020knowing, xu-etal-2020-position, wu-etal-2020-grid} originate from Semeval Challenges \citep{pontiki-etal-2014-semeval, pontiki2015semeval, pontiki2016semeval}, which covers only two domains\footnote{They have four sub-datasets. One sub-dataset is from the laptop domain, and the others are from the restaurant domain.}, i.e., restaurant and laptop. A dataset with only two domains can not show diversified domain discrepancy and therefore, can not measure the performance of cross-domain ASTE accurately and comprehensively.
    % The effectiveness of cross-domain ASTE methods can not be validated sufficiently with only two domains\WZ{look for some citations}.

    \item \textbf{Monotonous reviews.} Reviews in the existing datasets (e.g., 14Lap) are usually short sentences as shown in Figure \ref{fig:intro-cmp}(a). Besides, we explore sentence complexity by counting the number of n-grams in the part-of-speech (POS) sequences. Figure \ref{fig:intro-cmp}(b) demonstrates that reviews in 14Lap are of simple sentence patterns. Moreover, triplets in these datasets exclude implicit aspect terms, which account for a large proportion. Models trained on such monotonous datasets tend to overfit to specific review patterns, which leads to performance drop when applied to real scenarios.
    % \HY{overfit may be overclaimed, => However, reviews in real-world scenarios are often complex and diverse (e.g., Electronics reviews from the Amazon website).}
    % \XT{有cross-dataset的实验结果证明，应该可以说overfit}
    % As shown in Figure (\ref{fig:intro-length}) and (\ref{fig:intro-pos}), reviews in the existing datasets (e.g. 14Lap) are usually short and simple instances. 
\end{itemize}

To advance the research of cross-domain ASTE, we construct a manually annotated dataset Multi-Domain ASTE (\textbf{\datasetwb}) and design a detailed annotation procedure to ensure the quality of \datasetwb. Compared with the existing datasets, \dataset contains data from more domains and the reviews are more diversified, e.g., various lengths, assorted sentence patterns, and triplets with both implicit and explicit aspect terms.

To investigate the challenges in cross-domain ASTE, we adopt some representative models and conduct extensive experiments based on \dataset in multiple settings. Then we provide future directions for cross-domain ASTE. Specifically, we conclude that \dataset is a more challenging dataset than previous datasets through the in-domain results. For the single-source domain adaptation, we conduct detailed experiments to analyze the challenges introduced by the cross-domain setting. Empirical results indicate that reducing domain discrepancy can be a promising direction for cross-domain ASTE. Moreover, we investigate the negative transfer in the multi-source cross-domain setting and observe that most of the negative transfer comes from dissimilar source-target pairs, which indicates that domain similarity can be a domain selection guideline for future multi-source cross-domain research.
% For the cross-dataset experiments\footnote{e.g., train on \citet{xu-etal-2020-position} and test on \datasetwb.}, we conclude that models trained from \dataset have better generalizability than those trained from the prior dataset. 

The main contributions of this paper can be summarized as follows: 
\begin{itemize}
    \item To the best of our knowledge, we are the first to investigate cross-domain ASTE.
    \item We construct a new manually annotated dataset \dataset that covers eight domains and contains diversified reviews, which is challenging for the cross-domain ASTE task. 
    \item We carry out extensive experiments in multiple scenarios and provide promising directions for future research.
\end{itemize}






==> chapters/2_related_work.tex <==
\section{Related Work}
\noindent\textbf{ASTE.} Current ASTE datasets originate from SemEval Challenge datasets \citep{pontiki-etal-2014-semeval, pontiki2015semeval, pontiki2016semeval}. The SemEval Challenge datasets provide the aspect terms and the corresponding sentiments, covering domains from restaurant and laptop. Based on the datasets,  \citet{fan2019target} annotate the aspect-opinion pairs. 
To provide more detailed information about the review text, the researchers resort to extracting sentiment triplets from the review, i.e., aspect term, opinion term, and sentiment polarity. \citet{peng2020knowing}  and \citet{wu-etal-2020-grid}  align the datasets of \citet{fan2019target} and original SemEval Challenge datasets to build the ASTE datasets. Based on \citet{peng2020knowing}, \citet{xu-etal-2020-position} find that they do not contain cases where one opinion term is associated with multiple aspects. \citet{xu-etal-2020-position} refine the dataset and release a new version. As mentioned in Section \ref{sec:intro}, these datasets cover limited domains with monotonous reviews. However, our dataset covers more domains and diversified reviews, and therefore, can be better applied to real-world scenarios\footnote{The aspect quadruple datasets \citep{cai-etal-2021-aspect, zhang-etal-2021-aspect-sentiment} can also be transformed into aspect triplets. We omit the comparison with them since they share almost the same data origination with the existing triplet dataset.}.
% In summary, all the ASTE datasets originate from the SemEval Challenges, which contains only two domains, i.e., restaurant and laptop. 

% \XT{remove description for each method.}
% Corresponding\WZ{Representative} solutions for ASTE can be divided into three categories: tagging-based \citep{peng2020knowing,xu-etal-2020-position, zhang-etal-2020-multi-task, wu-etal-2020-grid, li2019unified, xu-etal-2021-learning}, MRC-based \citep{chen2021bidirectional, mao2021joint}, and generation-based \cite{zhang2021towards, yan-etal-2021-unified, fei2021nonautoregressive, mukherjee-etal-2021-paste, hsu2021semantics}. 
% The tagging-based methods employ a sequence or grid tagging framework to solve the ASTE task. For example, \citet{xu-etal-2021-learning} introduce a span-level interaction model (Span-ASTE) to learn interactions between the aspect and opinion spans.  
% The MRC-based method constructs queries for a review sentence. For example, \citet{mao2021joint} design two queries to first extract the aspects and then predict the opinion and sentiment polarity toward the aspect. \citet{chen2021bidirectional} further advance this idea and propose a bidirectional MRC (BMRC) model. One direction sequentially extracts the aspect-oriented triplets. And the other sequentially identifies the opinion-oriented triplets.
% The generation-based method transforms the ASTE task into a sequence generation problem. For example, \citet{zhang2021towards} directly output the triplets in the plain text given a review.  \citet{yan-etal-2021-unified} adapt BART \citep{lewis-etal-2020-bart} as a pointer network to generate the index of the aspect terms, opinion terms, and sentiments.

Corresponding solutions for ASTE can be divided into three categories: tagging-based \citep{peng2020knowing, xu-etal-2020-position, zhang-etal-2020-multi-task, wu-etal-2020-grid, li2019unified, xu-etal-2021-learning}, MRC-based \citep{chen2021bidirectional, mao2021joint}, and generation-based \citep{zhang2021towards, yan-etal-2021-unified, fei2021nonautoregressive, mukherjee-etal-2021-paste, hsu2021semantics}. 
The tagging-based method employs a sequence or grid tagging framework to extract the aspect and opinion terms, then combine them to predict the sentiment. 
The MRC-based method constructs a specific query for each factor in the triplets and extracts them through the answer to the query.
The generation-based method employs sequence-to-sequence (seq2seq) models and transforms the ASTE task into a sequence generation problem. Then it decodes the triplets through a specifically designed algorithm. In this study, we employ some representative models in the three categories and explore \dataset in multiple settings.


% However, these methods heavily rely on a large amount of labeled data. Since annotating triplets in a given sentence is time-consuming, obtaining massive training data for every domain is impractical. We propose to explore the ASTE task in the cross-domain setting. 


\noindent\textbf{Cross-domain SA and Cross-domain ABSA.} 
Existing domain adaptation methods mainly focus on sentence analysis (SA) or aspect-based sentiment analysis (ABSA). Most of them can be grouped into feature-based and instance-based domain adaptation. Feature-based methods focus on learning domain-invariant features. For example, \citet{blitzer2007biographies} introduce a structural correspondence learning algorithm to link the source and target domains. 
\citet{ganin2016domain} leverage domain adversarial learning to learn features invariant to domain discrepancy. Instance-based methods concentrate on re-weight training data in the source domain. \citet{li-etal-2012-cross} apply re-weighting on the source domain instances based on pseudo-labeled data. Based on the two methods, \citet{gong2020unified} combine feature-based and instance-based methods to achieve better domain adaptation.

The above methods all focus on sentence or aspect-level classification tasks. However, ASTE is a structural extraction task, which extracts more detailed sentimental information in the review. Existing domain adaptation methods for SA or ABSA can not be well adapted to cross-domain ASTE. 
% \XT{cross-domain ASTE is a structural extraction task, existing methods .. }can not be adapted to ..There is no specifically designed method for cross-domain ASTE. \XT{remove AT} In this study, we integrate adversarial training, a dominant solution in domain adaptation, with current ASTE methods. And we conduct extensive experiments to provide suggestions for future research.

==> chapters/3_dataset.tex <==
\input{tables/data_statistics.tex}
\input{tables/data_comparison.tex}
% \input{tables/data_comparison_new.tex}

\section{Dataset}
\label{sec:dataset}

% To better investigate the cross-domain ASTE task, we construct a Multi-domain ASTE dataset (\datasetwb). 
This section will first introduce the data collection and annotation process of Multi-domain ASTE dataset (\datasetwb).
To better investigate and understand \datasetwb, then we show the statistics and characteristics of \datasetwb.

\subsection{Collection}
\dataset is derived from the Amazon dataset \footnote{\url{https://nijianmo.github.io/amazon/index.html\#sample-review}.} \citep{ni2019justifying}, which is publicly available. It is a large crawl of product reviews from Amazon. 
This dataset contains 233.1 million unique reviews covering 29 domains. 
We sample eight more common domains of e-commerce and randomly sample reviews from each domain.
% a portion of the dataset and annotate the sentiment triplets. 


\subsection{Annotation}
\label{sec:annotation}
% We follow the train-trial-annotate-check procedure to ensure the quality of annotation.
% 14 workers (annotators) are employed to annotate and 4 workers (verifiers) are employed to do the quality-assurance sampling (QA sampling). Both are paid according to the number of annotations.
% First\XT{enumerate it}, we train all workers on the labeling guidelines. Then they enter the trial phase. During this phase, workers \XT{annotator/verifier?} try to understand the task and improve the annotation quality, meanwhile,\XT{} we check all the annotations and give feedback.
% Once they reach 95\% accuracy in labeling, they will proceed to the official phase. 
% During the official phase\XT{official?}, verifiers sample 20\% annotations every day. If the accuracy of an annotator is lower than 95\%, then all the data of that annotator for that day will be re-checked.

Following \citet{peng2020knowing,xu-etal-2020-position,wu-etal-2020-grid}, we annotate \textit{(aspect term, opinion term, sentiment polarity)} triplets for each instance.
Every instance is a complete review, which may include multiple sentences.
\textit{Aspect term} refers to a part or an attribute of products or services.
Sometimes, the aspect term may not appear explicitly in the instance, i.e., implicit aspect \citep{poria2014rule}. We keep the triplets with implicit aspects.
An \textit{opinion term} is a word or phrase that expresses opinions or attitudes towards aspects.
\textit{Sentiment polarity} is the sentiment type of the opinion term, which is divided into three categories: positive, negative, and neutral.
It is worth noting that one aspect is associated with multiple opinions and vice versa. 

We employ 14 workers (annotators) to annotate and 4 workers (verifiers) to do the quality-assurance sampling (determine whether the annotation is correct). Both are paid according to the number of annotations. We follow the train-trial-annotate-check procedure to ensure the quality of annotation.
(1) \textit{train}: We train all workers on this task.
(2) \textit{trial}: All workers try to understand the task and annotate the data. Meanwhile, we check all the annotations and give feedback. Once they reach 95\% accuracy in labeling, they proceed to the next phase.
(3) \textit{annotate}: Annotators annotate the data every day. 
(4) \textit{check}: Verifiers sample 20\% annotations every day. If the accuracy of an annotator is lower than 95\%, then all the data of that annotator for that day will be re-done until reach the accuracy requirement. Otherwise, we keep the annotations.

\subsection{Statistics and Characteristics}
The basic statistics of \dataset are shown in Table \ref{tab:statistics}. \dataset covers eight domains.
% i.e., Electronics, Fashion, Beauty, Home, Book, Pet, Toy, and Grocery. 
According to the number of reviews in the Amazon dataset, we select Electronics, Fashion, Beauty, and Home as source domains because they are the leading fields of e-commerce, and there are massive reviews for these domains. We select Book, Pet, Toy, and Grocery as target domains because they have fewer reviews and are very different from each other. For the source domains, we annotate more data and divide data into training, development, and test sets with a ratio of 7: 1: 2. For the target domains, we annotate fewer data and divide target data into development and test sets with a ratio of 1: 2 since we study the unsupervised domain adaptation setting.
% Among the eight domains, we select \XT{} Electronics, Fashion, Beauty, and 
% % 选择领域差异较大的四个作为源领域，然后选择领域差异多样化的作为目标领域。
% Home as source domains and annotate more data. Then we select Book, Pet, Toy, and Grocery as target domains and annotate fewer data. For the source domains, we divide data into training, development, and test sets with a ratio of 7: 1: 2. 
% For the target domains, we divide target data into development and test sets with a ratio of 1: 2 since we study more challenging unsupervised domain adaptation. 

In Table \ref{tab:cmp}, we further compare our dataset with existing representative datasets \citep{peng2020knowing, wu-etal-2020-grid, xu-etal-2020-position} in ASTE. Take the dataset of \citet{xu-etal-2020-position} for example, the number of instances and domains in our dataset is about 1.3 and 4 times of  \citet{xu-etal-2020-position},  respectively. And the review length in our dataset is about 3.6 times of \citet{xu-etal-2020-position}. Moreover, \dataset contains both implicit and explicit aspects while the others only annotate explicit aspects. Besides, we represent the sentence complexity of our reviews by counting the n-grams in part-of-speech (POS) sequences and dependency parsing (DP) trees \footnote{For the DP tree, we treat the parent node and child node as neighbors.}. The comparison results show that the number of n-grams of POS and DP trees in \dataset is significantly higher than that of other datasets, and the number of 4-grams is about 3 times that of other datasets, which indicates the reviews in \dataset are more diverse and complex.

The characteristics of \dataset can be summarized as follows:
\begin{itemize}
    \item \textbf{Multiple domains.} \dataset contains eight domains which is much more than previous datasets. It can provide more transfer pairs and enable more sufficient research on the cross-domain ASTE task.
    \item \textbf{Diversified reviews.} Reviews in \dataset are of various lengths and assorted sentence patterns. Moreover, the triplets contain both implicit and explicit aspect terms. All of them make the ASTE task more challenging.
\end{itemize}


% In Table \ref{tab:cmp}, we further compare our dataset with existing representative datasets \citep{peng2020knowing, wu2020grid, xu2020position} in ASTE. First, we include \textbf{more domains} and instances in \datasetwb. The number of instances and domains in our dataset is about 1.3 and 4 times of previous datasets, respectively.  Second, the reviews in \dataset are \textbf{diversified}. The review length in our dataset is about 3.6 times the previous one. Besides, we investigate the expression diversity of our reviews by counting the n-grams in part-of-speech (POS) sequences and dependency parsing (DP) trees \footnote{For the DP tree, we treat the parent node and child node as neighbors.}. The comparison results show that the number of n-grams of POS and DP trees in \dataset is significantly higher than that of other datasets. And the number of 4-grams is even more than twice that of other datasets.
% Moreover, \dataset contains both \textbf{implicit and explicit aspects} while the others only annotate explicit aspects. 



==> chapters/4_formulation.tex <==
\section{Problem Formulation}
\noindent\textbf{ASTE.} Given an instance $\mathbf{x} = \{w_1, w_2,..., w_n\}$,  consisting of $n$ words, the goal of the ASTE task is to extract a set of sentiment triplets $\mathbf{y} = \{(a_1, o_1, s_1), ..., (a_i, o_i, s_i),...\}$ from the instance $\mathbf{x}$, where $a$, $o$ and $s$ denote the aspect term, opinion term, and sentiment polarity, respectively. 

% % TODO: 用大写S表示源领域，大写T表示目标领域，N表示样本数量
\noindent\textbf{Cross-Domain ASTE.}  We focus on the unsupervised domain adaptation setting, in which manual annotations are only available in the source domain. Formally, given one or multiple set of source domain samples $D^S = \{(\mathbf{x}_i^s, \mathbf{y}_i^s\}_{i=1}^{N^s}$ \HY{$S={S_1...S_n}$, where n denotes the number of source domain?, or introduce the multi-source setting later}
and target domain samples $D^T = \{(\mathbf{x}_i^t\}_{i=1}^{N^t}$. The target data label is unknown. For the single-source cross-domain research, the source domain samples come from a single domain while 
% Thus, we are interested in training a network using labeled source domain data $D^S$ and unlabeled target domain data $D^T$ to make accurate predictions on the target domain. 

==> chapters/5_models.tex <==
\section{Approaches}
% ASTE 是什么，方法， 2.cross-domain ASTE是什么，方法
In this section, we describe modeling approaches that we benchmark on \datasetwb. Because we are the first to address the cross-domain ASTE task, there is no specifically designed method for ASTE in the cross-domain setting. Therefore, we employ current representative methods for ASTE and incorporate some methods with adversarial training, a common solution in domain adaptation.

\subsection{Baseline Models For ASTE}
Traditional methods toward ASTE can be grouped into three categories: tagging-based, MRC-based, and generation-based. In this study, we select one or two representative models from the three different frameworks.

\noindent\textbf{BMRC}: BMRC \citep{chen2021bidirectional} employs the MRC framework. Considering that one triplet can derive from either an aspect term or an opinion term, they propose to address the ASTE task bidirectionally. Specifically, one direction sequentially extracts the aspect term, opinion term, and sentiment. And the other direction sequentially identifies the opinion term, aspect term, and sentiment. 
% By merging the extraction results from the two directions, they can identify triplets more comprehensively. 

\noindent\textbf{Span-ASTE}: Span-ASTE \citep{xu-etal-2021-learning} is a tagging-based method. It first extracts aspect terms and opinion terms by predictions of all the spans. Then it obtains the aspect-opinion pairs by performing Cartesian Product \citep{warner1990modern} on the extracted aspect and opinion terms. Finally, it identifies the sentiments by classifying the pairs. 

\noindent\textbf{BART-ABSA}: BART-ABSA \citep{yan-etal-2021-unified} is a generation-based method. It generates the start and end position index of the aspect term, the start and end position index of the opinion term, and the index of sentiment polarity sequentially. 

\noindent\textbf{GAS}: \citep{zhang2021towards} utilize T5 model  \citep{raffel2020exploring} to generate sentiment triplets in plain text. For the first example in Figure \ref{fig:intro-example}, given the input sentence, GAS generates triplets "\textit{(wire holders, pretty flimsy, negative), (wire holders, work, positive)}" in the decoder.

% \input{tables/in_domain}
\input{tables/main_results}

\subsection{Adversarial Training For Cross-domain}
The above models are all designed for the in-domain setting. We integrate BMRC and Span-ASTE with adversarial training\footnote{We exclude BART-ABSA and GAS because domain adversarial training is not applicable to generative models.}, a dominant method in the cross-domain setting. Adversarial training learns domain-invariant features by a min-max game between the feature generator and domain discriminator \citep{tang2020adversarial}. We describe where to apply domain discriminator as follows.

\noindent\textbf{BMRC + AT}: For BMRC, the aspect terms and opinion terms are extracted by classifying the token representations, and the sentiment polarities are obtained by classifying the [CLS] representations. Therefore, we apply a domain discriminator on the token and [CLS] features. In this way, we can learn discriminative features by classifiers of the ASTE task and learn domain-invariant features by the domain discriminator induced by adversarial training.

\noindent\textbf{Span-ASTE + AT}: Span-ASTE first obtains the token representation through the encoder. Then it combines the start and end token representations for each span and obtains span representations. By classification of the span representations, it extracts all the aspect and opinion terms. Then it conducts Cartesian Product on the aspect and opinion terms and identifies the sentiment polarities of the aspect-opinion pairs. Because all the representations originate from the token representations, We apply adversarial learning to the token representations as in BMRC + AT methods.


==> chapters/6_experiment/fig_analyse_ins.tex <==
% \subsection{Challenges from ASTE}
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/analysis/length.pdf}
         \caption{F1 scores on reviews of different lengths.}
         \label{fig:analyse-length}
     \end{subfigure}
        \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/analysis/pos.pdf}
         \caption{F1 scores on reviews of different numbers of POS 2-grams.}
         \label{fig:analyse-pos}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/analysis/imp.pdf}
         \caption{F1 scores on reviews of different aspect types.}
         \label{fig:analyse-imp}
     \end{subfigure}
        \caption{F1 scores on different review lengths, different numbers of POS 2-grams, and different aspect types. The results are average F1 scores on 16 transfer pairs. We can conclude that long reviews, complex sentences, and implicit aspect terms make \dataset more challenging. }
        \label{fig:analyse-ins}
\end{figure*}


==> chapters/6_experiment/fig_case_study.tex <==
% \subsection{Case Study}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/case.pdf}
    \caption{Case Study. The golden labels are highlighted in the original text.}
    \label{fig:case_study}
\end{figure*}

% In Figure \ref{fig:case_study}, we further conduct a case study on predictions of Span-ASTE. The first example shows that Span-ASTE may not extract domain-specific opinion terms, e.g. \textit{Well written}. The second example shows that: (1) Span-ASTE may not identify some domain-specific aspect terms, e.g., \textit{writing, wording, expressions}. The reason is that these aspect terms differs greatly from the aspect terms in the beauty domain.  (2) Span-ASTE may mismatch the aspect and opinion, e.g., \textit{(expressions, beautiful, positive)} (3) Span-ASTE fail to capture long-distance dependence, e.g., \textit{(descriptions, enjoyed, positive)}. We can observe from the triplets of the third example that: Span-ASTE may mismatch the aspect and opinion terms which is a pair but in a short distance. e.g., \textit{(shipping, cannot be beat, POS)}.

==> chapters/6_experiment/in_domain.tex <==
\subsection{In-Domain Results}
Table \ref{tab:in-domain} shows the overall comparison results on in-domain ASTE where the training data and test data are from the same domain. We can observe that: (1) Span-ASTE performs the best on \dataset and achieves comparable results with GAS on $\mathcal{D}_X$. (2) The performance of the four models on the dataset of \citet{xu-etal-2020-position} is better than on \datasetwb, which indicates that \dataset introduces more challenges to the ASTE research empirically. More analysis can be seen in Appendix \ref{sec:app-in-domain}. (3) Among the four domains in \datasetwb, models perform consistently the best in the fashion domain and the worst in the beauty domain.

==> chapters/6_experiment/main.tex <==
\section{Experiment Results}
In this section, we explore \dataset in multiple scenarios, i.e., in-domain, single-source cross-domain, and multi-source cross-domain. 

\input{chapters/6_experiment/in_domain}

% figure & table
\input{tables/multi_source}
\input{chapters/6_experiment/fig_analyse_ins}
\input{chapters/6_experiment/fig_corr}
\input{tables/cross_4to1}
\input{chapters/6_experiment/fig_case_study}


\input{chapters/6_experiment/single_source}
% \input{chapters/6_experiment/analysis_instance}
% \input{chapters/6_experiment/analysis_domain}


\input{chapters/6_experiment/multi_source}



==> chapters/6_experiment/multi_source.tex <==
\subsection{Multi-Source Cross-Domain Results}
We conduct multi-source cross-domain experiments when the number of source domains ranges from 2 to 4. The results of transferring all four source domains to the target domain are shown in Table \ref{tab:4-1}. We can observe that transferring four domains to each target domain is consistently better than transferring a single source domain to the target domain. Then we investigate the results when transferring from two or three source domains to the book domain. We present part of the results in Table \ref{tab:multi-source} due to space limitation. We find the situation of negative transfer. For example, B + H $\to$ K > B + E + H $\to$ K, F + H $\to$ K > E + F + H $\to$ K. It indicates that simply combining multiple sources to a single source domain may wash out informative characteristics of individual domains and lead to negative transfer \citep{guo-etal-2018-multi}. Therefore, an advanced multi-source domain adaptation strategy is required for cross-domain ASTE research.

==> chapters/6_experiment/set_up.tex <==

\subsection{Experimental Setup}
% \noindex\textbf{Datasets.} In order to evaluate the effectiveness of our dataset, we conduct experiments on \datasetwb, Restaurant-14 (R), and Laptop-14 (L) datasets from \citet{xu2020position}. For \datasetwb, we treat electronics (E), Fashion (F), Beauty (B), and Home (H) as source domains, Book (K), Pet (P), Toy (T), and Grocery (G) as target domains. For restaurant and laptop datasets, we conduct experiments on R$\to$L and L$\to$R. 

\noindent\textbf{Implementation Details.} We implement all the models via Pytorch 1.10.0 with a piece of V100. We use AdamW optimizer \citep{loshchilov2017decoupled}. 

\noindent\textbf{Evaluation Metric.} In our study, we employ Micro-F1 to measure the performance of different approaches. Only an exact match could be counted as correct. All experiments are repeated 5 times with random seeds from 1 to 5. 

==> chapters/6_experiment/single_source.tex <==
\subsection{Single-Source Cross-Domain Results}\label{sec:exp-single}
We report the Micro-F1 scores of various methods on 16 transfer pairs of \dataset in Table \ref{tab:main-results}. From the table we can make the following observations: 
(1) The results are consistently lower than those in Table \ref{tab:in-domain}. 
(2) The performances vary a lot when transferring from different source domains to a target domain. e.g. Micro-F1 score of Span-ASTE on H$\to$ T is 47.60, which is 6.41 higher than that on B$\to$T.
(3) Span-ASTE generally performs the best compared with all the baseline models.
(4) Adversarial training hurts the performance of BMRC and Span-ASTE.

Then we further analyze the above observations through detailed experiments. And answer the following questions:


\noindent\textbf{What is the challenge in \dataset dataset? } We propose this question because of the consistent performance drop in Observation 1. Then we answer this question by comparing the performance under different sentence lengths, sentence complexity, and aspect types as shown in Figure \ref{fig:analyse-ins}. 
\begin{itemize}
    \item \textbf{Length.} As shown in Figure (\ref{fig:analyse-length}), we categorize the instance by its length and test the model for each category. We can observe that the longer the instance, the worse the model performance. Since \dataset contains reviews of various lengths, this characteristic introduces more challenges to the task.
    \item \textbf{Sentence Complexity.} We represent sentence complexity by the number of 2-grams in the POS sequence of the review text. Then we explore the relation between the extraction performance and sentence complexity. Figure (\ref{fig:analyse-pos}) shows that the performance decreases with the sentence complexity increasing.
    % In Figure (\ref{fig:analyse-pos}), we investigate the performance of the model when the number of triplets ranges from 1 to 7. We find that the performance of the model first increases and then decreases with the number of triplets growing. \XT{TBD}
    % \XT{reasons}
    \item \textbf{Aspect Types.} In Figure (\ref{fig:analyse-imp}), we compare the Micro-F1 results of triplets with implicit and explicit aspects. The results suggest that the implicit aspect is harder for the model than the explicit aspect. 
    \dataset includes both implicit and explicit aspects. It makes \dataset more challenging.
    % Because the implicit aspect can refer to any attribute of the product which introduces ambiguity in the extraction process. 
\end{itemize}
We can conclude that long reviews, complex sentence, and implicit aspects make \dataset a challenging dataset. 

\noindent\textbf{What is challenge in the cross-domain setting?} Observation 2 indicates the performance gap when transferring from different domains. So we analyze the challenges from the cross-domain setting by investigating the relationship between transfer performance and domain similarity.
We fix the number of training data for each source domain (to alleviate the impact of data volume) and obtain their performance on the target domain. Then we compute the domain similarity by the vocabulary overlaps as in \citet{liu2021crossner}. The results are shown in Figure \ref{fig:corr}. We observe that the Span-ASTE performance and domain similarity have a Pearson correlation coefficient \citep{benesty2009pearson} of 0.52, which means that cross-domain performance and domain similarity are positively correlated. Therefore, reducing the domain discrepancy may be a promising direction for cross-domain ASTE. It can be seen that more transfer pairs enable more sufficient analysis in the cross-domain setting which can not be done with only two domains.


\noindent\textbf{Why Span-ASTE outperforms GAS?} In the in-domain experiments on $\mathcal{D}_X$, Span-ASTE achieves comparable results with GAS. But it outperforms GAS in \datasetwb. We attribute this reversal to the various instance lengths in \datasetwb. As shown in Figure (\ref{fig:analyse-length}), Span-ASTE achieves comparable performance when the instance length ranges from 1 to 100. But when the instance length exceeds 100, Span-ASTE outperforms GAS by a large margin. We analyze the cases and find that GAS tends to misspell or generate a phrase that never appears when the review is long. For the last example in Figure \ref{fig:case_study}, \textit{"how they work well"} never appears in the original text. And Span-ASTE does not have this problem because it just identifies the start token and end token for aspect or opinion terms.

\noindent\textbf{Why adversarial training hurts the performance?} Comparing the results of BMRC v.s. BMRC + AT and Span-ASTE v.s. Span-ASTE + AT, we can conclude that adversarial training hurts the performance in cross-domain ASTE. We attribute the performance drop to the loss of domain-specific information. For the ASTE task, each domain has specific aspect terms and opinion terms. Simply learning domain-invariant features may lead to the loss of domain-specific information. As shown in Figure \ref{fig:case_study}, Span-ASTE + AT can not identify domain-specific aspect term \textit{"clear plastic adapters"} and domain-specific opinion terms \textit{"a little brittle"} in the first example.

==> chapters/6_experiment_1205/cross-dataset.tex <==
\noindent\textbf{Cross-dataset Results.}
% To compare the \XT{} between \citet{xu-etal-2020-position} and \dataset, 
% we conduct cross-dataset experiments based on Span-ASTE due to the state-of-the-art performance in the cross-domain setting.
% Then we report the F1 scores of Span-ASTE for cross-dataset when transferring from \dataset to \citet{xu-etal-2020-position} and from \citet{xu-etal-2020-position} to \dataset in Table \ref{tab:maste2xu} and \ref{tab:xu2maste}, respectively. The results demonstrate a considerable performance drop when transferring from \citet{xu-etal-2020-position} to \datasetwb. The results conform with our intuition that models trained from the existing datasets tend to overfit to specific review patterns and will lead to performance drop when migrated to real scenarios. And the higher results in Table \ref{tab:maste2xu} also demonstrate the better generalizability of \dataset over \citet{xu-etal-2020-position}. \XT{can we describe the dataset with generalizability?}
To compare the generalizability of models trained from \citet{xu-etal-2020-position} and \datasetwb, 
we conduct cross-dataset experiments based on Span-ASTE, the state-of-the-art model in the cross-domain setting, and compare the results with the in-domain results in Table \ref{tab:in-domain} in the appendix.
F1 scores for cross-dataset are shown in Table \ref{tab:maste2xu} and \ref{tab:xu2maste} regarding transferring from \dataset to \citet{xu-etal-2020-position} and from \citet{xu-etal-2020-position} to \datasetwb, respectively. The results reveal the better generalizability of models trained from \datasetwb. For example, the F1 score for transferring from 14Res in \citet{xu-etal-2020-position} to Electronics in \dataset is 14.18, while the F1 score for transferring from Electronics in \dataset to 14Res in \citet{xu-etal-2020-position} is 39.81. 
Compared with the in-domain result, the cross-dataset result transferring from electronics is reduced by 45\%, while the result transferring from 14Res is reduced by 70\%. It demonstrates better generalizability of models trained from \datasetwb.
% The results demonstrate a considerable performance drop when transferring from \citet{xu-etal-2020-position} to \datasetwb. The results conform with our intuition that models trained from the existing datasets tend to overfit to specific review patterns and will lead to performance drop when migrated to real scenarios. And the higher results in Table \ref{tab:maste2xu} also demonstrate the better generalizability of \dataset over \citet{xu-etal-2020-position}. \XT{can we describe the dataset with generalizability?}


==> chapters/6_experiment_1205/formulation.tex <==
\subsection{ASTE Formulation}
Given an instance $\mathbf{x} = \{w_1, w_2,..., w_n\}$,  consisting of $n$ words, the goal of the ASTE task is to extract a set of sentiment triplets $\mathbf{y} = \{(a_1, o_1, s_1), ..., (a_i, o_i, s_i),...\}$ from the instance $\mathbf{x}$, where $a$, $o$ and $s$ denote the aspect term, opinion term, and sentiment polarity, respectively. 
We evaluate the extraction performance by F1 scores, and only exact matching can be considered correct. 
% % TODO: 用大写S表示源领域，大写T表示目标领域，N表示样本数量
% \noindent\textbf{Cross-Domain ASTE.}  We focus on the unsupervised domain adaptation setting, in which manual annotations are only available in the source domain. Formally, given one or multiple set of source domain samples $D^S = \{(\mathbf{x}_i^s, \mathbf{y}_i^s\}_{i=1}^{N^s}$ \HY{$S={S_1...S_n}$, where n denotes the number of source domain?, or introduce the multi-source setting later}
% and target domain samples $D^T = \{(\mathbf{x}_i^t\}_{i=1}^{N^t}$. The target data label is unknown. For the single-source cross-domain research, the source domain samples come from a single domain while 
% Thus, we are interested in training a network using labeled source domain data $D^S$ and unlabeled target domain data $D^T$ to make accurate predictions on the target domain. 
% \HY{multi-source formulation TBD}

==> chapters/6_experiment_1205/main.tex <==
\section{Experiments}
To better evaluate cross-domain ASTE on \datasetwb, we conduct extensive experiments in multiple settings. This section will first introduce the ASTE formulation and different experiment setups, then describe the approaches employed in the experiments, and finally show the results in single-source cross-domain, multi-source cross-domain, and cross-dataset settings. For these results, we give an in-depth analysis in Section \ref{sec:analysis}.

\input{chapters/6_experiment_1205/formulation.tex}

\input{chapters/6_experiment_1205/set_up.tex}

\input{tables/main_results}
\input{tables/cross_dataset.tex}


\input{chapters/6_experiment_1205/models.tex}

\subsection{Results}
\label{sec:results}

\input{chapters/6_experiment_1205/single-source.tex}



\input{chapters/6_experiment/fig_analyse_ins.tex}
\input{tables/multi_source.tex}
\input{chapters/6_experiment/fig_corr.tex}

\input{chapters/6_experiment_1205/multi-source.tex}

\input{chapters/6_experiment_1205/cross-dataset.tex}

==> chapters/6_experiment_1205/models.tex <==
% \section{Approaches}
% % ASTE 是什么，方法， 2.cross-domain ASTE是什么，方法
% In this section, we describe modeling approaches that we benchmark on \datasetwb. Because we are the first to address the cross-domain ASTE task, there is no specifically designed method for ASTE in the cross-domain setting. Therefore, we employ current representative methods for ASTE and incorporate some methods with adversarial training, a common solution in domain adaptation.

\subsection{Models}
This section describes  approaches that we benchmark on \datasetwb. Because we are the first to study the cross-domain ASTE task, there is no specifically designed method for ASTE in the cross-domain setting. Therefore, we employ current representative methods for ASTE and incorporate some of them with adversarial training \citep{ganin2016domain}, a dominant solution in domain adaptation.

\noindent\textbf{Baseline Models For ASTE.} 
We select some representative models from the tagging-based, MRC-based, and generation-based frameworks. 

\begin{itemize}
    \item \textit{Span-ASTE} \citep{xu-etal-2021-learning}: a tagging-based method. It explicitly considers the span interaction between the aspect and opinion terms.
    \item \textit{BMRC} \citep{chen2021bidirectional}: a MRC-based method. It  extracts aspect-oriented triplets and opinion-oriented triplets. Then it obtains the final results by merging the two directions. 
    \item  \textit{BART-ABSA} \citep{yan-etal-2021-unified}: a generation-based method. It employs a pointer network and generates indices of the aspect term, opinion term, and sentiment polarity sequentially. 
    \item \textit{GAS} \citep{zhang2021towards}: a generation-based method. It transforms the ASTE tasks into a text generation problem.
\end{itemize} 



\noindent\textbf{Adversarial Training For Cross-domain ASTE.}
 We integrate Span-ASTE and BMRC with adversarial training and describe where to apply the domain discriminator as follows:
 % \footnote{We exclude BART-ABSA and GAS because domain adversarial training is not applicable to generative models. \XT{search for it}}. 有相关工作把对抗加到生成方法里
 % Adversarial training learns domain-invariant features by a min-max game between the feature generator and domain discriminator \citep{tang2020adversarial}. 

 \begin{itemize}
    \item \textit{BMRC + AT}: We apply a domain discriminator on the token and [CLS] features. In this way, we can learn discriminative features by classifiers of the ASTE task and domain-invariant features by the domain discriminator induced by adversarial training.
    \item \textit{Span-ASTE + AT}: Because the extraction is based on the prediction of the span and pair representation. Both of them originate from the token representation. Therefore, we apply adversarial learning to the token representations as in the BMRC + AT model.
\end{itemize}

% \begin{itemize}
%     \item \textit{BMRC + AT}: For BMRC, the aspect terms and opinion terms are extracted by classifying the token representations, and the sentiment polarities are obtained by classifying the [CLS] representations. Therefore, we apply a domain discriminator on the token and [CLS] features. In this way, we can learn discriminative features by classifiers of the ASTE task and domain-invariant features by the domain discriminator induced by adversarial training.
%     \item \textit{Span-ASTE + AT}: Span-ASTE first obtains the token representation through the encoder. Then it combines the start and end token representations for each span and obtains span representations. By classification of the span representations, it extracts all the aspect and opinion terms. Then it conducts Cartesian Product on the aspect and opinion terms and identifies the sentiment polarities of the aspect-opinion pairs. Because all the representations originate from the token representations, We apply adversarial learning to the token representations as in BMRC + AT methods.
% \end{itemize}


==> chapters/6_experiment_1205/multi-source.tex <==
\noindent\textbf{Multi-source Cross-domain Results.}
We conduct multi-source cross-domain experiments when the number of source domains ranges from 2 to 4 in Table \ref{tab:multi-source}. 
(1) From the results of transferring from all four source domains to different target domains, we can observe that transferring four domains to each target domain is consistently better than transferring a single source domain to the target domain. 
(2) We find the situation of negative transfer when transferring from two or three source domains. For example, B + H $\to$ Book > B + E + H $\to$ Book, F + H $\to$ Grocery > E + F + H $\to$ Grocery. It indicates that some source domains have drastically different distributions from the target domain. And transferring from these domains could harm the learning of the target domain \citep{guo-etal-2018-multi}. Therefore, domain selection may be a promising direction for future multis-source cross-domain ASTE research.
% It indicates that simply combining multiple sources to a single source domain may wash out informative characteristics of individual domains and lead to negative transfer \citep{guo-etal-2018-multi}. \XT{refine, long->short} 

==> chapters/6_experiment_1205/set_up.tex <==
\subsection{Setups}
We conduct experiments with the following training/test setups:
\begin{itemize}

    \item  \textit{Single-source Cross-domain}: we train the models with data from a single-source domain and test them on a target domain.

    \item \textit{Multi-source Cross-domain}: we train the models with data from multiple source domains and test them on a target domain.

    \item \textit{Cross-dataset}: we train and test the models on different datasets, e.g., train with data from \citet{xu-etal-2020-position} and test on \datasetwb.

\end{itemize}
Detailed experiment settings are shown in Appendix \ref{sec:app-exp-settings}.



==> chapters/6_experiment_1205/single-source.tex <==
\noindent\textbf{Single-source Cross-domain Results.}\label{sec:exp-single}
Table \ref{tab:main-results} reports the F1 scores of various methods on 16 transfer pairs of \datasetwb. Here we present the summary of the results. (1) The results on the 16 transfer pairs are consistently low, indicating that \dataset is a challenging dataset. 
(2) The performances vary a lot when transferring from different source domains to a target domain. e.g. F1 score of Span-ASTE on Home$\to$ Toy is 47.60, which is 6.41 higher than that on Beauty$\to$Toy. 
(3) Span-ASTE generally performs the best compared with all the baseline models.
(4) Adversarial training hurts the performance of BMRC and Span-ASTE.
We present an in-depth analysis in section \ref{sec:analysis}. 

==> chapters/6_experiment_1225/main.tex <==
\section{Experiment Settings}
To better evaluate cross-domain ASTE on \datasetwb, we conduct extensive experiments in multiple settings. This section will first introduce the ASTE formulation, then present different experiment setups, and finally describe the approaches employed in the experiments.
\input{chapters/6_experiment_1205/formulation.tex}
\input{chapters/6_experiment_1225/set_up.tex}
\input{chapters/6_experiment_1205/models.tex}

==> chapters/6_experiment_1225/set_up.tex <==
\subsection{Setups}
We conduct experiments with the following training/test setups:
\begin{itemize}
    \item \textit{In-domain}: we train and test the models with data from the same domain.
    
    \item  \textit{Single-source Cross-domain}: we train the models with data from a single-source domain and test them on a different target domain.

    \item \textit{Multi-source Cross-domain}: we train the models with data from multiple source domains and test them on a different target domain.

    % \item \textit{Cross-dataset}: we train and test the models on different datasets, e.g., train with data from \citet{xu-etal-2020-position} and test on \datasetwb.

\end{itemize}
Detailed experiment settings are shown in Appendix \ref{sec:app-exp-settings}.



==> chapters/7_analysis/cross-domain.tex <==
\subsection{Cross-domain Setting Analysis}
 Table \ref{tab:main-results} demonstrates the performance gap when transferring from different domains. To further analyze the reason, we carry out Pearson Correlation Analysis \citep{benesty2009pearson} to investigate the relationship between transfer performance and domain similarity.
Specifically, we first fix the number of training data for each source domain to alleviate the impact of data volume. Secondly, we obtain their performance on the target domain. Then we compute the domain similarity by the vocabulary overlaps \citep{liu2021crossner}. Vocabulary for each domain is created by considering the top 1k most frequent words except stopwords. The results are shown in Figure \ref{fig:corr}. We observe that the Span-ASTE performance and domain similarity have a Pearson correlation coefficient  of 0.52, which means that cross-domain performance and domain similarity are positively correlated. Therefore, reducing the domain discrepancy may be a promising direction for cross-domain ASTE. 
% It can be seen that more transfer pairs enable sufficient analysis in the cross-domain setting, which can not be done with only two domains.


==> chapters/7_analysis/dataset.tex <==
\subsection{Challenges in \dataset}
\label{sec:analyse-dataset}
Compared with ASTE results in previous works \citep{xu-etal-2021-learning}, we can observe the performance drop in Table \ref{tab:main-results}. So we further analyze the challenges in \dataset by comparing the performance under different review lengths, sentence complexity, and aspect types as shown in Figure \ref{fig:analyse-ins}.  All the results are average F1 scores of 16 transfer pairs in the single-source cross-domain setting.
\begin{itemize}
    \item \textbf{Length.} As shown in Figure \ref{fig:analyse-ins}(a), we categorize the instance by its length and test the model for each category. We can observe that the longer the instance, the worse the model performance. Since \dataset contains reviews of various lengths, this characteristic introduces more challenges to the task.
    \item \textbf{Sentence Complexity.} We represent sentence complexity by the number of 2-grams in the POS sequence of the review text. Then we explore the relationship between extraction performance and sentence complexity. Figure \ref{fig:analyse-ins}(b) shows that the performance decreases with the sentence complexity increases.
    % In Figure (\ref{fig:analyse-pos}), we investigate the performance of the model when the number of triplets ranges from 1 to 7. We find that the performance of the model first increases and then decreases with the number of triplets growing. \XT{TBD}
    % \XT{reasons}
    \item \textbf{Aspect Types.} In Figure \ref{fig:analyse-ins}(c), we compare the F1 results of triplets with implicit and explicit aspect terms. The results suggest that the implicit aspect term is harder for the model than the explicit one. 
    \dataset includes both implicit and explicit aspects terms. It makes \dataset more challenging.
    % Because the implicit aspect can refer to any attribute of the product which introduces ambiguity in the extraction process. 
\end{itemize}
We can conclude that long reviews, complex sentences, and implicit aspect terms make \dataset a challenging dataset. 

==> chapters/7_analysis/main.tex <==
\section{Analysis}
\label{sec:analysis}
To better understand \dataset and the cross-domain ASTE task, we conduct analyses from multiple perspectives based on Span-ASTE, the state-of-the-art method in cross-domain experiments. We first analyze challenges introduced by \datasetwb. Then we focus on the cross-domain performance gap and find the performance correlates well with the domain similarity. Finally, we make detailed comparisons across strong baselines on representative cases. Some analysis results shed light on multiple promising ways to boost cross-domain ASTE tasks for future research.

\input{chapters/7_analysis/dataset.tex}


\input{chapters/6_experiment/fig_case_study.tex}
\input{chapters/7_analysis/cross-domain.tex}

\input{chapters/7_analysis/model_cmp.tex}

==> chapters/7_analysis/model_cmp.tex <==

\subsection{Model Comparison}
\noindent\textbf{With AT v.s. Without AT.} Comparing the results of BMRC v.s. BMRC + AT and Span-ASTE v.s. Span-ASTE + AT, we can conclude that adversarial training hurts the performance in cross-domain ASTE. We attribute the performance drop to the loss of domain-specific information. For the ASTE task, each domain has specific aspect terms and opinion terms. Simply learning domain-invariant features may lead to the loss of domain-specific knowledge. For the first example in Figure \ref{fig:case_study}, Span-ASTE + AT can not identify domain-specific aspect term \textit{"clear plastic adapters"} and domain-specific opinion term \textit{"a little brittle"} in the first example.

\noindent\textbf{Span-ASTE v.s. GAS.} Prior works \citep{xu-etal-2021-learning, zhang2021towards} show that Span-ASTE achieves comparable results with GAS on \citet{xu-etal-2020-position}. But it outperforms GAS in \datasetwb. We attribute this reversal to the various instance lengths in \datasetwb. As shown in Figure \ref{fig:analyse-ins}(a), Span-ASTE achieves comparable performance when the instance length is less than 100. But when the instance length exceeds 100, Span-ASTE outperforms GAS by a large margin. We analyze the cases and find that GAS tends to misspell or generate a phrase that never appears when the review is long. For the last example in Figure \ref{fig:case_study}, \textit{"how they work well"} never appears in the original text. And Span-ASTE does not have this problem because it just identifies the start token and end token for aspect or opinion terms.



==> chapters/7_conclusion.tex <==
\section{Conclusion and Future Directions}
We propose \datasetwb, a manually-annotated ASTE dataset collected from Amazon. Compared with the existing ASTE dataset, \dataset contains reviews of various lengths, assorted sentence patterns, more aspect types and covers more domains. We implement some representative models based on the three frameworks of ASTE. Then we explore the dataset in multiple scenarios, i.e., in-domain, single-source cross-domain, and multi-source cross-domain. For the in-domain experiments, we compare the results between existing datasets and \dataset and find that the review length, sentence complexity, and the aspect type in the triplets make \dataset a challenging dataset. For the single-source cross-domain experiments, we conduct extensive analyses to explore the cross-domain ASTE task. From the cross-domain perspective, we observe that domain similarity and cross-domain performance are positively correlated. Therefore, reducing the domain discrepancy can be a promising direction for cross-domain ASTE. For the multi-source domain-adaptation results, we find that most of the negative transfer comes from dissimilar source-target pairs, pointing out that domain similarity can be a domain selection guideline for future research.
% we find that some domains may cause negative transfer, pointing out that advanced domain selection methods are necessary for multi-source research. 

==> chapters/7_results_1225/in-domain.tex <==
\subsection{In-domain}
\label{sec:app-in-domain}
We present the overall in-domain experimental results in Table \ref{tab:in-domain}, and then conduct a detailed analysis to investigate the challenges of \datasetwb. 
% Through this analysis, we aim to gain a better understanding of the limitations of current approaches on this challenging dataset. 
Finally, we compare the best-performing models to provide insights for future work in this area.

\paragraph{Challenges of \datasetwb.} We present an analysis of the challenges introduced by \dataset for the ASTE task. Results from the in-domain experiments, reported in Table \ref{tab:in-domain}, show a decline in performance when compared to results on the dataset of \citet{xu-etal-2020-position}. To further investigate the challenges of \datasetwb, we conducted an analysis of the performance under different review lengths, sentence complexity, and aspect types.

\begin{itemize}
    \item \textbf{Length.} In Figure \ref{fig:analyse-indomain-ins}(a), we present the relationship between the review length and the model performance on \datasetwb. Results indicate that the performance of the models decreases as the length of the review increases. This trend highlights the challenge that the diversity in review length poses to the task, as MASTE contains reviews of various lengths, which poses a significant challenge to the models.


    \item \textbf{Sentence Complexity.} We quantify the sentence complexity by calculating the number of 2-grams in the POS sequence of the review text. An analysis of the relationship between extraction performance and sentence complexity is conducted. As shown in Figure \ref{fig:analyse-indomain-ins}(b), we observe a decline in performance with an increase in sentence complexity. This highlights the challenges posed by diverse sentence structures present in \datasetwb.
    
    \item \textbf{Aspect Types.} In Figure \ref{fig:analyse-indomain-ins}(c), we present an analysis of the performance of models on triplets with implicit and explicit aspect terms. The results indicate that the extraction of implicit aspect terms is more challenging for the models than that of explicit aspect terms. The inclusion of both implicit and explicit aspect terms in \dataset makes it more challenging for ASTE.
    
\end{itemize}
We can conclude that long reviews, complex sentences, and implicit aspect terms make \dataset a challenging dataset.

\paragraph{Model Comparison.}
 Prior works \citep{xu-etal-2021-learning, zhang2021towards} show that Span-ASTE achieves comparable results with GAS on \citet{xu-etal-2020-position}. But it outperforms GAS in \datasetwb. 
We attribute this reversal to the various instance lengths in \datasetwb. GAS is a generation-based method that outputs the sentiment triplets word by word. When the reviews are long, GAS is inclined to forget the original text and  misspell it or generate a phrase that never appears. Span-ASTE is a tagging-based method that only identifies the start and end tokens for the aspect and opinion terms. 
 For the last example in Figure \ref{fig:case_study}, GAS outputs \textit{"how they work well"} as an opinion term that never appears in the original text. 

==> chapters/7_results_1225/main.tex <==
\input{tables/in_domain.tex}
\input{chapters/7_results_1225/fig-in-domain.tex}
\section{Results}

This section presents a thorough analysis of the challenges of the \dataset dataset and the ASTE task, with the aim of providing a better understanding of these challenges and suggesting promising directions for future research. We first present the results of our experiments in different settings. Then we conduct a comprehensive analysis to investigate the challenges of the dataset and the task, highlighting the limitations of current approaches on this challenging dataset. Finally, we provide insights into the limitations of current approaches and suggest directions for future research in this area.

\input{chapters/7_results_1225/in-domain.tex}

\input{tables/main_results}
\input{chapters/7_results_1225/single-source.tex}
\input{chapters/6_experiment/fig_corr.tex}
\input{chapters/6_experiment/fig_case_study.tex}

\input{tables/multi_source.tex}
\input{chapters/7_results_1225/multi-source.tex}



==> chapters/7_results_1225/multi-source.tex <==
\subsection{Multi-source Cross-domain}
\noindent\textbf{Results.} We conduct multi-source cross-domain experiments when the number of source domains ranges from 2 to 4 in Table \ref{tab:multi-source}. 
(1) From the results of transferring from all four source domains to different target domains, we can observe that transferring four domains to each target domain is consistently better than transferring a single source domain to the target domain. 
(2) We find the situation of negative transfer when transferring from two or three source domains. For example, F + H $\to$ Book > E + F + H $\to$ Book, F + H $\to$ Grocery > B + F + H $\to$ Grocery. 

\noindent\textbf{Analysis.} 
Negative transfer indicates that some source domains have drastically different distributions from the target domain. And transferring from these domains could harm the learning of the target domain \citep{guo-etal-2018-multi}. We further compare the results with the domain similarity in Figure \ref{fig:corr}(b) and find that most of the negative transfer comes from the most dissimilar source-target pairs. It demonstrates that domain similarity can be a domain selection guideline for future multi-source cross-domain research.
% Therefore, domain selection may be a promising direction for future multi-source cross-domain ASTE research.
% It indicates that simply combining multiple sources to a single source domain may wash out informative characteristics of individual domains and lead to negative transfer \citep{guo-etal-2018-multi}. \XT{refine, long->short} 

==> chapters/7_results_1225/single-source.tex <==
\subsection{Single-source Cross-domain}\label{sec:exp-single}
\noindent\textbf{Results.} Table \ref{tab:main-results} reports the F1 scores of various methods on 16 transfer pairs of \datasetwb. Here we present some observations. (1) The results on the 16 transfer pairs are lower than those in the in-domain setting, indicating that cross-domain ASTE is a challenging task. 
(2) The performances vary a lot when transferring from different source domains to a target domain. e.g. F1 score of Span-ASTE on Home$\to$ Toy is 47.60, which is 6.41 higher than that on Beauty$\to$Toy. 
(3) Adversarial training hurts the performance of BMRC and Span-ASTE.
(4) Span-ASTE generally performs the best compared with all the baseline models.

% We present an in-depth analysis in section \ref{sec:analysis}. 

 \noindent\textbf{Model performance v.s. Domain similarity.} Table \ref{tab:main-results} demonstrates the performance gap when transferring from different domains. To further analyze the reason, we carry out Pearson Correlation Analysis \citep{benesty2009pearson} to investigate the relationship between transfer performance and domain similarity.
Specifically, we first fix the number of training data for each source domain to alleviate the impact of data volume. Secondly, we obtain the model performance on the target domain. Then we compute the domain similarity by the vocabulary overlaps \citep{liu2021crossner}. Vocabulary for each domain is created by considering the top 1k most frequent words except stopwords. The results are shown in Figure \ref{fig:corr}. We observe that the Span-ASTE performance and domain similarity have a Pearson correlation coefficient  of 0.52, which means that cross-domain performance and domain similarity are positively correlated. It indicates that large domain discrepancy is the challenge for the cross-domain ASTE task. Therefore, reducing the domain discrepancy may be a promising direction for cross-domain ASTE. 

% \noindent\textbf{With AT v.s. Without AT.} Comparing the results of BMRC v.s. BMRC + AT and Span-ASTE v.s. Span-ASTE + AT, we can conclude that adversarial training hurts the performance in cross-domain ASTE. We attribute the performance drop to the loss of domain-specific information. For the ASTE task, each domain has specific aspect terms and opinion terms. Simply learning domain-invariant features may lead to the loss of domain-specific knowledge. For the first example in Figure \ref{fig:case_study}, Span-ASTE + AT can not identify domain-specific aspect term \textit{"clear plastic adapters"} and domain-specific opinion term \textit{"a little brittle"} in the first example.

\noindent\textbf{With AT v.s. Without AT.} Comparing the results of BMRC v.s. BMRC + AT and Span-ASTE v.s. Span-ASTE + AT, we can conclude that adversarial training hurts the performance in cross-domain ASTE. We attribute the performance drop to feature collapse \citep{tang2020discriminative} induced by adversarial training, which focuses on learning domain-invariant features while ignoring the discriminability of each category. This issue is more serious in the ASTE task because it requires more fine-grained discrimination for three factors. Therefore, simply learning domain-invariant features may cause feature collapse and lead to the loss of domain-specific knowledge. For the first example in Figure \ref{fig:case_study}, Span-ASTE + AT can not identify domain-specific aspect term \textit{"clear plastic adapters"} and domain-specific opinion term \textit{"a little brittle"} in the first example.



==> chapters/8_limitations.tex <==
\section*{Limitations}
We analyze the limitations of this study from the following perspectives:
\begin{itemize}
    % \item The \dataset dataset is based on English reviews so it is limited to English, as most of the existing ASTE datasets. Future work can include more languages into the research.
    \item The ASTE task extracts the sentiment triplets from a review, while the Aspect Sentiment Quad Prediction (ASQP) task adds an aspect category based on the triplets and provides more comprehensive information. Future work can take the aspect category into consideration.
    \item All the models are evaluated by F1, in which only exact matching can be considered correct. This metric can not differentiate between partially matching and completely mismatching and is not the best choice for a challenging dataset like \datasetwb. Future work can include some partially matching metrics for this task.
    \item There is no specifically designed method for cross-domain ASTE. But we analyze the challenges of this task in detail. We are planning to design a new method for cross-domain ASTE based on the analysis results.
\end{itemize}


==> chapters/main.tex <==

\input{chapters/0_abstract}
\input{chapters/1_intro}
\input{chapters/2_related_work}
\input{chapters/3_dataset}

% \input{chapters/6_experiment_1205/main}
% \input{chapters/7_analysis/main}

\input{chapters/6_experiment_1225/main}
\input{chapters/7_results_1225/main}
\input{chapters/7_conclusion}
\input{chapters/8_limitations.tex}
\bibliography{anthology,custom}
\bibliographystyle{acl_natbib}

\appendix

\input{chapters/8_appendix/main.tex}

==> chapters_0110/0_abstract.tex <==
\begin{abstract}
    Aspect  Sentiment Triplet Extraction (ASTE) is widely applied to various applications. However, existing datasets for ASTE are limited in their ability to represent real-world scenarios, hindering the advancement of research in this area. In this paper, we introduce a new dataset, named \datasetwb, which is manually annotated to better fit real-world scenarios by providing more diverse and realistic reviews for the task. The dataset includes various lengths, assorted sentence patterns, more aspect types, and more domains than existing datasets. We conduct extensive experiments in multiple settings to evaluate the performance of the \dataset dataset and the ASTE task. Empirical results demonstrate that \dataset is a more realistic and challenging dataset for ASTE. Based on the detailed analysis on the experiments, we discusss multiple promising directions for future research.
    % We found that the performance of existing methods declines significantly on \datasetwb, indicating that it is a challenging dataset. We also observe a positive correlation between transfer performance and domain similarity in the single-source cross-domain setting. Additionally, we investigate negative transfer in the multi-source cross-domain setting and observe that most of it comes from dissimilar source-target pairs, which suggests that domain similarity can be a useful guideline for future multi-source cross-domain research. 

\end{abstract}

==> chapters_0110/1_intro.tex <==

\section{Introduction}
\label{sec:intro}

Aspect sentiment triplet extraction \citep[ASTE;][]{peng2020knowing}, a fine-grained task in sentiment analysis \citep{hussein2018survey}, has attracted considerable interest recently \citep{peng2020knowing, xu-etal-2020-position}.  The objective of this task is to extract sentiment triplets, comprising of an aspect term, an opinion term, and a sentiment polarity, from a given review. As depicted in Figure \ref{fig:intro-example}, an example of a sentiment triplet is ({\textit{"curly cord"}, \textit{"hate"}, \textit{NEG}}), representing a \textit{negative} sentiment towards the aspect term \textit{"curly cord"} using the opinion term {\textit{"hate"}} .

\begin{figure}[htbp] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering
\includegraphics[width=0.45\textwidth]{figures/intro-example.pdf} 
\caption{An Example for the ASTE task. The terms highlighted in blue are aspect terms. The terms in orange are opinion terms. The words in green are sentiment polarities. "NULL" denotes the implicit aspect.} 
\label{fig:intro-example} %用于文内引用的标签
\end{figure}


A well-trained ASTE model can be widely applied to various real-world scenarios \citep{zhang2022survey}. One specific application is the analysis of customer reviews on E-commerce platforms. Through this technique, organizations are able to gain valuable insights that can aid in the improvement of products or services and the development of more effective marketing campaigns.


However, it is well known that real-world scenarios tend to be complex and existing datasets \citep{peng2020knowing, xu-etal-2020-position, wu-etal-2020-grid} are limited to represent real-world scenarios, limiting the advancement of the research on ASTE. To further illustrate this limitation, a comparison was conducted between the dataset presented in \citet{xu-etal-2020-position} and our dataset, as presented in Figure \ref{fig:intro-cmp}. The comparison results demonstrate that existing datasets primarily consist of \textit{short reviews} characterized by \textit{simple sentence patterns}. These limitations in the datasets impede the generalizability of the ASTE model to accurately represent real-world scenarios.

\input{figures/fig-data-cmp.tex}


In order to enhance the generalizability of the ASTE model to real-world scenarios, we  created a new dataset, named Diversified Multi-domain ASTE (\datasetwb), which was manually annotated to provide a more diverse and realistic set of reviews for the task. The key characteristics of \dataset can be summarized as follows: (1) \textbf{Various Length}: \dataset covers reviews of various lengths, ranging from 1 to 250. (2) \textbf{Assorted sentence patterns}: \dataset includes reviews with a variety of sentence structures, enabling the model to handle the complexity and diversity of real-world scenarios. (3) \textbf{More aspect types}: \dataset  includes triplets annotated with both implicit and explicit aspect terms, providing the model with a more comprehensive understanding of the entity being discussed. (4) \textbf{More domains}: \dataset covers eight domains, enabling more comprehensive research in ASTE like single-source and multi-source domain adaptation.
To summarize, These characteristics allow the model to better handle the variability present in the data encountered in actual usage.
 
In order to thoroughly investigate the challenges introduced by \dataset and identify  promising directions for future ASTE research, we implement several representative methods and empirically evaluate \dataset under multiple settings, including in-domain, single-source cross-domain, and multi-source cross-domain. Specifically, in-domain result shows that the performance of current models declines significantly on \datasetwb. And the analysis results suggest that \textit{future works can focus on dealing with long reviews, complex sentences and implicit aspect terms}. In the single-source domain adaptation setting, we analyse the factors that impact transfer performance and observe a positive correlation between transfer performance and domain similarity, which suggests that \textit{reducing domain discrepancy can be a future direction}.\XT{corr or AT?} Furthermore, we investigate the phenomenon of negative transfer in the multi-source cross-domain setting and find that the majority of negative transfer arises from dissimilar source-target pairs. This suggests that \textit{domain similarity may be a useful guideline for selecting domains} in future multi-source cross-domain research. Overall, the evaluation results of \dataset on multiple settings provide a deeper understanding of the challenges and future directions for ASTE research.

The main contributions of this paper can be summarized as follows: 
\begin{itemize}
    \item We present a new dataset, \datasetwb, which is manually annotated to provide more diverse and realistic reviews for the ASTE task.
    \item We carry out extensive experiments in multiple scenarios and provide promising directions for future research.
    \item \XT{what can we provide to the community?}
\end{itemize}






==> chapters_0110/2_related_work.tex <==
\section{Related Work}
\subsection{ASTE Datasets}
Current datasets \citep{peng2020knowing, xu-etal-2020-position, wu-etal-2020-grid} for the task of ASTE share the a common origin and are constructed through similar processes. Specifically, they originate from SemEval Challenge datasets \citep{pontiki-etal-2014-semeval, pontiki2015semeval, pontiki2016semeval}, which provide aspect terms and corresponding sentiments for reviews in the domains of restaurant and laptop.  Based on the datasets,  \citet{fan2019target} annotate the aspect-opinion pairs. 
To provide more detailed information about the review text, researchers resort to extracting sentiment triplets from the review, i.e., aspect term, opinion term, and sentiment polarity. \citet{peng2020knowing}  and \citet{wu-etal-2020-grid}  construct the ASTE datasets by aligning the aspect terms between the datasets of \citet{fan2019target} and original SemEval Challenge datasets. However, as noted by \citet{xu-etal-2020-position}, the dataset of \citet{peng2020knowing} does not contain cases where one opinion term is associated with multiple aspects. \citet{xu-etal-2020-position} subsequently refined the dataset and released a new version. 

However, all of these datasets contains reviews of limited diversity from only two domains. Additionally, they all require aspect terms to align the aspect-sentiment pair and aspect-opinion pair, thus they do not include implicit aspect terms\citep{poria2014rule}. Our dataset, \datasetwb, addresses these limitations by providing a more diverse set of reviews covering more domains and annotate both implicit and explicit aspect terms, making it better suited for real-world scenarios \footnote{\citep{cai-etal-2021-aspect, zhang-etal-2021-aspect-sentiment} can also be transformed into aspect triplets. We omit the comparison with them since they share almost the same data origination with the existing triplet dataset.}.

\subsection{ASTE Methods}
Corresponding solutions for ASTE can be divided into three categories: tagging-based \citep{peng2020knowing, xu-etal-2020-position, zhang-etal-2020-multi-task, wu-etal-2020-grid, li2019unified, xu-etal-2021-learning}, MRC-based \citep{chen2021bidirectional, mao2021joint}, and generation-based \citep{zhang2021towards, yan-etal-2021-unified, fei2021nonautoregressive, mukherjee-etal-2021-paste, hsu2021semantics}. 
The tagging-based method employs a sequence or grid tagging framework to extract the aspect and opinion terms, then combine them to predict the sentiment. 
The MRC-based method constructs a specific query for each factor in the triplets and extracts them through the answer to the query.
The generation-based method employs sequence-to-sequence (seq2seq) models and transforms the ASTE task into a sequence generation problem. Then it decodes the triplets through a specifically designed algorithm. In this study, we employ some representative models in the three categories and explore \dataset in multiple settings.


% However, these methods heavily rely on a large amount of labeled data. Since annotating triplets in a given sentence is time-consuming, obtaining massive training data for every domain is impractical. We propose to explore the ASTE task in the cross-domain setting. 


==> chapters_0110/3_dataset.tex <==
\input{tables/data_statistics.tex}
% \input{tables/data_comparison.tex}
\input{tables/data_comparison_new.tex}

\section{Dataset}
\label{sec:dataset}

% To better investigate the cross-domain ASTE task, we construct a Multi-domain ASTE dataset (\datasetwb). 
To construct a dataset that is more representative of real-world scenarios, we mannually annotate a new dataset, named Diversified Multi-domain ASTE (\datasetwb).  In this section, we first present a detailed description of the data collection and annotation process. Then we demonstrate the superiority of \datasetwb, through a comparison with previous datasets in terms of key statistics and characteristics.

\subsection{Collection}
The data collection process for \datasetwb is carried out in three stages:
(1) We selected the Amazon dataset as our primary source of data due to its large volume of reviews from various regions around the world, which aligns with the goal of creating a dataset that is more representative of real-world scenarios.
(2) We selected four of the most popular domains from the Amazon dataset (Appendix \ref{sec:app-dataset}), and randomly sampled a portion of the data for annotation.
(3) In the third stage, to further enable comprehensive exploration of ASTE like domain adaptation settings, we additionally sampled four additional domains and annotated a smaller portion of the data for testing in domain adaptation settings.

\subsection{Annotation}
\label{sec:annotation}

\paragraph{Simplified Annotation guidelines\footnote{Due to space limitation, we present detailed labeling guideline in Appendix \ref{sec:app-guideline}.}.}Following \citet{peng2020knowing,xu-etal-2020-position,wu-etal-2020-grid}, we annotate \textit{(aspect term, opinion term, sentiment polarity)} triplets for each instance.
Every instance is a complete review, which may include multiple sentences.
\textit{Aspect term} refers to a part or an attribute of products or services.
Sometimes, the aspect term may not appear explicitly in the instance, i.e., implicit aspect \citep{poria2014rule}. We keep the triplets with implicit aspects.
An \textit{opinion term} is a word or phrase that expresses opinions or attitudes towards aspects.
\textit{Sentiment polarity} is the sentiment type of the opinion term, which is divided into three categories: positive, negative, and neutral.
It is worth noting that one aspect is associated with multiple opinions and vice versa. 

\paragraph{Annotation Process.} 
In order to ensure the quality of the annotation process, we employed 14 workers (annotators) to perform the annotation and 4 workers (verifiers) to perform quality-assurance sampling. Both groups were compensated based on the number of annotations completed. The annotation process was carried out using a train-trial-annotate-check procedure.
(1) \textit{Train}: All the workers were trained on the task of annotation.
(2) \textit{Trial}: All the workers annotated a small portion of the data to familiarize themselves with the task and to receive feedback on their annotations. The workers were required to reach 95\% accuracy in labeling before proceeding to the next phase.
(3) \textit{Annotate}: The annotators were responsible for annotating the data on a daily basis.
(4) \textit{Check}: The verifiers sampled 20\% of the annotations each day to ensure accuracy. If the accuracy of an annotator was found to be below 95\%, the data annotated by that worker for that day would be re-done until the accuracy requirement was met. Otherwise, the annotations were accepted.

\subsection{Statistics and Characteristics}
% The basic statistics of \dataset are shown in Table \ref{tab:statistics}. \dataset covers eight domains. According to the number of reviews in the Amazon dataset, we select Electronics, Fashion, Beauty, and Home as source domains because they are the leading fields of e-commerce, and there are massive reviews for these domains. We select Book, Pet, Toy, and Grocery as target domains because they have fewer reviews and are very different from each other. 
% For the source domains, we annotate more data and divide data into training, development, and test sets with a ratio of 7: 1: 2. For the target domains, we annotate fewer data and divide target data into development and test sets with a ratio of 1: 2 since we study the unsupervised domain adaptation setting.
% Among the eight domains, we select \XT{} Electronics, Fashion, Beauty, and 
% % 选择领域差异较大的四个作为源领域，然后选择领域差异多样化的作为目标领域。
% Home as source domains and annotate more data. Then we select Book, Pet, Toy, and Grocery as target domains and annotate fewer data. For the source domains, we divide data into training, development, and test sets with a ratio of 7: 1: 2. 
% For the target domains, we divide target data into development and test sets with a ratio of 1: 2 since we study more challenging unsupervised domain adaptation. 

To provide a deeper understanding of our proposed dataset, we present a series of statistics and characteristics in this section.

\paragraph{Various lengths.} Figure \ref{fig:intro-cmp}(a) illustrates the comparison of review length between \citet{xu-etal-2020-position} \datasetwb. We find that \dataset contains reviews of various lengths. And Table \ref{tab:cmp} demonstrates that the average length of \dataset is 3.6 times that of \citet{xu-etal-2020-position}. 
\paragraph{Assorted sentence patterns.} We quantify the sentence complexity of our reviews by counting the n-grams in part-of-speech (POS) sequences and dependency parsing (DP) trees \footnote{For the DP tree, we treat the parent node and child node as neighbors.}.  Figure \ref{fig:intro-cmp}(b) shows the comparison of POS 2-grams between \citet{xu-etal-2020-position} and \datasetwb. The results indicate that \dataset contains reviews with assorted sentence patterns.  And Table \ref{tab:cmp} shows that the number of n-grams of POS and DP trees in \dataset is significantly higher than those of other datasets, with the number of 4-grams being about 3 times that of other datasets. This indicates that the reviews in \dataset are more diverse and complex.

\paragraph{More aspect types.} Table \ref{tab:cmp} shows that \dataset not only contains more explicit aspect terms than existing datasets but also includes annotations of implicit aspect terms, which constitute a larger proportion. This provides a more comprehensive understanding of the target being discussed.
\paragraph{More domains.} Table \ref{tab:cmp} illustrates that our dataset comprises four times the number of domains compared to existing datasets. Furthermore, the first four domains presented in Table \ref{tab:statistics}, which are characterized by a larger amount of annotated data, represent leading fields in e-commerce platforms (Appdenix \ref{sec:app-dataset}), providing a more realistic representation of popular topics. Additionally, we include an additional four domains with less annotated data to enable a more comprehensive analysis of the domain adaptation setting.


In  summary, \dataset is a more realistic and diversified dataset, providing more challenges to the ASTE task.

% In Table \ref{tab:cmp}, we further compare our dataset with existing representative datasets \citep{peng2020knowing, wu2020grid, xu2020position} in ASTE. First, we include \textbf{more domains} and instances in \datasetwb. The number of instances and domains in our dataset is about 1.3 and 4 times of previous datasets, respectively.  Second, the reviews in \dataset are \textbf{diversified}. The review length in our dataset is about 3.6 times the previous one. Besides, we investigate the expression diversity of our reviews by counting the n-grams in part-of-speech (POS) sequences and dependency parsing (DP) trees \footnote{For the DP tree, we treat the parent node and child node as neighbors.}. The comparison results show that the number of n-grams of POS and DP trees in \dataset is significantly higher than that of other datasets. And the number of 4-grams is even more than twice that of other datasets.
% Moreover, \dataset contains both \textbf{implicit and explicit aspects} while the others only annotate explicit aspects. 



==> chapters_0110/4_experiment_settings/main.tex <==
\section{Experiment Settings}
To thoroughly evaluate \dataset and provide comprehensive suggestions for future ASTE research, we conduct massive experiments in various settings. This section will begin by providing an overview of the different experimental setups and then describe the models employed in the experiments in detail.
\input{chapters_0110/4_experiment_settings/set_up.tex}
\input{chapters_0110/4_experiment_settings/metric.tex}
\input{chapters_0110/4_experiment_settings/models.tex}

==> chapters_0110/4_experiment_settings/metric.tex <==
\subsection{Evaluation Metric} 
Following prior works \citep{xu-etal-2021-learning}, we employ the F1 score to measure the performance of different approaches. And only extract match can be considered correct.  All the experiment results are reported using the average of 5 random runs with random seeds from 0 to 4. 

==> chapters_0110/4_experiment_settings/models.tex <==
% \section{Approaches}
% % ASTE 是什么，方法， 2.cross-domain ASTE是什么，方法
% In this section, we describe modeling approaches that we benchmark on \datasetwb. Because we are the first to address the cross-domain ASTE task, there is no specifically designed method for ASTE in the cross-domain setting. Therefore, we employ current representative methods for ASTE and incorporate some methods with adversarial training, a common solution in domain adaptation.

\subsection{Models}
This section presents the various approaches that we evaluate on the \dataset dataset. We first introduce representative models for ASTE and employ them as our baseline models. 
Then for the single-source cross domain research, we utilize current methods for ASTE and integrate some of them with adversarial training \citep{ganin2016domain}, which is a widely-used technique for domain adaptation.

\paragraph{Baseline Models For ASTE.} 
We implement several representative models from various frameworks, including tagging-based, MRC-based, and generation-based frameworks. 

\begin{itemize}
    \item \textit{Span-ASTE} \citep{xu-etal-2021-learning}: a tagging-based method. It explicitly considers the span interaction between the aspect and opinion terms.
    \item \textit{BMRC} \citep{chen2021bidirectional}: a MRC-based method. It  extracts aspect-oriented triplets and opinion-oriented triplets. Then it obtains the final results by merging the two directions. 
    \item  \textit{BART-ABSA} \citep{yan-etal-2021-unified}: a generation-based method. It employs a pointer network and generates indices of the aspect term, opinion term, and sentiment polarity sequentially. 
    \item \textit{GAS} \citep{zhang2021towards}: a generation-based method. It transforms the ASTE tasks into a text generation problem.
\end{itemize} 

\paragraph{Baseline Models For Single-source Cross-domain.}
 We incorporate Span-ASTE and BMRC with adversarial training \citet[AT;][]{ganin2016domain}, a common strategy for domain adaptation. Specifically, we apply a domain discriminator on different features for each method:
 
 \begin{itemize}
    \item \textit{BMRC + AT}: We apply a domain discriminator on the token and [CLS] features. In this way, we can learn discriminative features by classifiers of the ASTE task and domain-invariant features by the domain discriminator induced by adversarial training.
    \item \textit{Span-ASTE + AT}: 
    As the extraction in this method is based on the prediction of the span and pair representation, which are derived from token representation, we apply adversarial learning to the token representations, similar to the BMRC + AT model.
\end{itemize}

% \begin{itemize}
%     \item \textit{BMRC + AT}: For BMRC, the aspect terms and opinion terms are extracted by classifying the token representations, and the sentiment polarities are obtained by classifying the [CLS] representations. Therefore, we apply a domain discriminator on the token and [CLS] features. In this way, we can learn discriminative features by classifiers of the ASTE task and domain-invariant features by the domain discriminator induced by adversarial training.
%     \item \textit{Span-ASTE + AT}: Span-ASTE first obtains the token representation through the encoder. Then it combines the start and end token representations for each span and obtains span representations. By classification of the span representations, it extracts all the aspect and opinion terms. Then it conducts Cartesian Product on the aspect and opinion terms and identifies the sentiment polarities of the aspect-opinion pairs. Because all the representations originate from the token representations, We apply adversarial learning to the token representations as in BMRC + AT methods.
% \end{itemize}


==> chapters_0110/4_experiment_settings/set_up.tex <==
\subsection{Setups}
We conduct a series of experiments under comprehensive training and testing setups:
\begin{itemize}
    \item \textit{In-domain}: we train and test the models with data from the same domain.
    
    \item  \textit{Single-source Cross-domain}: we train the models with data from a single-source domain and test them on a different target domain.

    \item \textit{Multi-source Cross-domain}: we train the models with data from multiple source domains and test them on a different target domain.

\end{itemize}
Detailed training details are shown in Appendix \ref{sec:app-exp-settings}.



==> chapters_0110/5_results/in-domain.tex <==
\subsection{In-domain}
\label{sec:app-in-domain}
 The overall in-domain experimental results are shown in Table \ref{tab:in-domain}. We first explore the limitations of all the models to better understand challenges introduced by \datasetwb. Then we compare two representative models to give suggestion for future research. 

\paragraph{Challenges of \datasetwb.} Results from the in-domain experiments, reported in Table \ref{tab:in-domain}, show a decline in performance when compared to results on existing datasets. To further investigate the challenges of \datasetwb, we conduct an analysis of the performance under different review lengths, sentence complexity, and aspect types. \XT{Does this analysis repeat too much?}

\begin{itemize}
    \item \textbf{Length. } In Figure \ref{fig:analyse-indomain-ins}(a), we show the relationship between the review length and the model performance on \datasetwb. Results indicate that the performance of the models decreases as the length of the review increases. This indicates that long reviews present a significant challenge for current models.
    \item \textbf{Sentence Complexity. } We quantify the sentence complexity by calculating the number of 2-grams in the part-of-speech (POS) sequence of the review text. Then we analyse  the relationship between extraction performance and sentence complexity. As shown in Figure \ref{fig:analyse-indomain-ins}(b), we observe a decline in performance with an increase in sentence complexity. This highlights the challenges posed by diverse sentence structures present in \datasetwb.
    \item \textbf{Aspect Types. } In Figure \ref{fig:analyse-indomain-ins}(c), we present an analysis of the performance of models on triplets with implicit and explicit aspect terms. The results demonstrate that the extraction of implicit aspect terms is more challenging for the models than that of explicit aspect terms. The inclusion of both implicit and explicit aspect terms in \dataset makes it more challenging for ASTE.  
\end{itemize}
We can conclude that long reviews, complex sentences, and implicit aspect terms make \dataset a challenging dataset.

\paragraph{Model Comparison.}
Prior works have demonstrated the state-of-the-art performance of GAS \citep{zhang2021towards}. 
However, as shown in Table \ref{tab:in-domain}, Span-ASTE outperforms GAS on \datasetwb. We conduct further analysis and discover that the reversal in performance can be attributed to the long instance lengths and complex sentence patterns presented in \datasetwb. As illustrated in Figure \ref{fig:analyse-indomain-ins}, GAS achieves comparable results when the reviews are short and simple, but its performance declines more sharply when encountering long and complex reviews in comparison to Span-ASTE. This can be attributed to the generation-based nature of GAS, which is prone to forgetting the original text and generating misspellings or phrases that do not appear in the review when dealing with longer reviews. In contrast, the tagging-based nature of Span-ASTE only identifies the start and end tokens for the aspect and opinion terms, which is less affected by the complexity and length of the reviews. This analysis provides insights for future generation-based methods: \textit{implementing a comparison algorithm between the generated output and the original input text and making modifications if they are mismatched.}
% As demonstrated in Figure 4, GAS outputs "how they work well" as an opinion term, which does not appear in the original text. \XT{change another figure}

==> chapters_0110/5_results/main.tex <==
\input{tables/in_domain.tex}
\input{chapters/7_results_1225/fig-in-domain.tex}
\section{Results}

This section presents a thorough analysis of the challenges of the \dataset dataset and the ASTE task, with the aim of providing a better understanding of these challenges and suggesting promising directions for future research. For each setting, we first present the results of our experiments. Then we conduct a comprehensive analysis to investigate the challenges of the dataset and the task, highlighting the limitations of current approaches. Finally, we provide suggestions for future research in this area.

\input{chapters_0110/5_results/in-domain.tex}

\input{tables/main_results}
\input{chapters_0110/5_results/single-source.tex}
\input{chapters/6_experiment/fig_corr.tex}
% \input{chapters/6_experiment/fig_case_study.tex}

\input{tables/multi_source.tex}
\input{chapters_0110/5_results/multi-source.tex}



==> chapters_0110/5_results/multi-source.tex <==
\subsection{Multi-source Cross-domain}
In this study, we conduct multi-source cross-domain experiments with the number of source domains varying from 2 to 4. Due to space limitation, we present part of the results in Table \ref{tab:multi-source}. Detailed results can be seen in Appendix \XT{}. Our results reveal instances of negative transfer. For example, F + H $\to$ Book > E + F + H $\to$ Book, F + H $\to$ Grocery > B + F + H $\to$ Grocery.

Negative transfer indicates that some source domains have drastically different distributions from the target domain. And transferring from these domains could harm the learning of the target domain \citep{guo-etal-2018-multi}. To further investigate the phenomenon of negative transfer, we conduct an analysis on the relationship between domain similarity and transfer performance. We further compare the results with the domain similarity in Figure \ref{fig:corr}(b). The results indicate that negative transfers are mostly observed when transferring from the source domains with the least similarity to the target domain. This suggests that domain similarity can serve as a useful guideline for selecting source domains in future multi-source cross-domain research.

==> chapters_0110/5_results/single-source.tex <==
\subsection{Single-source Cross-domain}\label{sec:exp-single}
We present the overall single-source cross-domain experimental results in Table \ref{tab:main-results} (Additional training details for adversarial training are shown in Appendix \ref{sec:app-adversarial}). We then conduct a correlation analysis to investigate the factors that impact transfer performance. Additionally, we analyze current domain adaptation strategies and provide insights for future research in this area.

% \noindent\textbf{Results.} Table \ref{tab:main-results} reports the F1 scores of various methods on 16 transfer pairs of \datasetwb. Here we present some observations. (1) The results on the 16 transfer pairs are lower than those in the in-domain setting, indicating that cross-domain ASTE is a challenging task. 
% (2) The performances vary a lot when transferring from different source domains to a target domain. e.g. F1 score of Span-ASTE on Home$\to$ Toy is 47.60, which is 6.41 higher than that on Beauty$\to$Toy. 
% (3) Adversarial training hurts the performance of BMRC and Span-ASTE.
% (4) Span-ASTE generally performs the best compared with all the baseline models.

% We present an in-depth analysis in section \ref{sec:analysis}. 

 \paragraph{Model performance v.s. Domain similarity.} 
 Table \ref{tab:main-results} reveals that performance varies significantly when transferring models from different source domains to a target domain,  e.g. F1 score of Span-ASTE on Home$\to$ Toy is 47.60, which is 6.41 higher than that on Beauty$\to$Toy. To gain insights into the factors that impact transfer performance, we conduct a Pearson Correlation Analysis  \citep{benesty2009pearson} on the relationship between model performance and domain similarity using Span-ASTE. Specifically, we fix the number of training data for each source domain to alleviate the impact of data volume. We measure domain similarity by computing vocabulary overlaps using the top 1k most frequent words in each domain, excluding stopwords. The results, as illustrated in Figure \ref{fig:corr}, show that there is a positive correlation (Pearson correlation coefficient of 0.52) between model performance and domain similarity. This indicates that large domain discrepancy is a significant challenge for the single-source cross-domain ASTE task. Therefore, future research in this area may focus on reducing domain discrepancy to improve performance in the cross-domain setting.


\paragraph{With AT v.s. Without AT.} 
We compare the performance of BMRC and BMRC + AT, as well as Span-ASTE and Span-ASTE + AT, as shown in Table \ref{tab:main-results}. The results indicate that  adversarial training (AT) has a negative impact on the performance of cross-domain ASTE. To understand the cause of this decline in performance, we visualize the representations learned by the models on the \XT{} test set when transferring from the \XT{} domain, as shown in Appendix \XT{}. \XT{prove this conjecture by case or figure?}Our analysis suggests that the decline in performance is likely due to feature collapse \citep{tang2020discriminative} induced by adversarial training. This occurs when the model focuses on learning domain-invariant features while ignoring the discriminability of each category. This issue is particularly pronounced in the ASTE task, as it requires fine-grained discrimination for three factors. Our findings suggest that simply learning domain-invariant features may lead to feature collapse and result in the loss of domain-specific knowledge. Future research in cross-domain ASTE could focus on \textit{developing methods that can learn domain-invariant features while maintaining the discriminability of each category.} 




==> chapters_0110/7_conclusion.tex <==
\section{Conclusion and Future Directions}
We propose \datasetwb, a manually-annotated ASTE dataset collected from Amazon. Compared with the existing ASTE dataset, \dataset contains reviews of various lengths, assorted sentence patterns, more aspect types and covers more domains. We implement some representative models based on the three frameworks of ASTE. Then we explore the dataset in multiple scenarios, i.e., in-domain, single-source cross-domain, and multi-source cross-domain. For the in-domain experiments, we compare the results between existing datasets and \dataset and find that the review length, sentence complexity, and the aspect type in the triplets make \dataset a challenging dataset. For the single-source cross-domain experiments, we conduct extensive analyses to explore the cross-domain ASTE task. From the cross-domain perspective, we observe that domain similarity and cross-domain performance are positively correlated. Therefore, reducing the domain discrepancy can be a promising direction for cross-domain ASTE. For the multi-source domain-adaptation results, we find that most of the negative transfer comes from dissimilar source-target pairs, pointing out that domain similarity can be a domain selection guideline for future research.
% we find that some domains may cause negative transfer, pointing out that advanced domain selection methods are necessary for multi-source research. 

==> chapters_0110/8_limitations.tex <==
\section*{Limitations}
We analyze the limitations of this study from the following perspectives:
\begin{itemize}
    % \item The \dataset dataset is based on English reviews so it is limited to English, as most of the existing ASTE datasets. Future work can include more languages into the research.
    \item The ASTE task extracts the sentiment triplets from a review, while the Aspect Sentiment Quad Prediction (ASQP) task adds an aspect category based on the triplets and provides more comprehensive information. Future work can take the aspect category into consideration.
    \item All the models are evaluated by F1, in which only exact matching can be considered correct. This metric can not differentiate between partially matching and completely mismatching and is not the best choice for a challenging dataset like \datasetwb. Future work can include some partially matching metrics for this task.
    \item There is no specifically designed method for cross-domain ASTE. But we analyze the challenges of this task in detail. We are planning to design a new method for cross-domain ASTE based on the analysis results.
\end{itemize}


==> chapters_0110/main.tex <==

\input{chapters_0110/0_abstract}
\input{chapters_0110/1_intro}
\input{chapters_0110/2_related_work}
\input{chapters_0110/3_dataset}

\input{chapters_0110/4_experiment_settings/main.tex}
\input{chapters_0110/5_results/main.tex}
\input{chapters_0110/7_conclusion}
\input{chapters_0110/8_limitations.tex}
\bibliography{anthology,custom}
\bibliographystyle{acl_natbib}

\appendix

\input{chapters_0110/8_appendix/main.tex}

==> chapters_0115/0_abstract.tex <==
\begin{abstract}
    Aspect  Sentiment Triplet Extraction (ASTE) is widely used in various applications. However, existing ASTE datasets are limited in their ability to represent real-world scenarios, hindering the advancement of research in this area. In this paper, we introduce a new dataset, named \datasetwb, which is manually annotated to better fit real-world scenarios by providing more diverse and realistic reviews for the task. The dataset includes various lengths, diverse expressions, more aspect types, and more domains than existing datasets. We conduct extensive experiments on \dataset in multiple settings to evaluate previous ASTE approaches. Empirical results demonstrate that \dataset is a more challenging ASTE dataset. Further analyses of in-domain and cross-domain settings provide promising directions for future research \footnote{Our dataset will be publicly available once accepted.}.
    % Based on the detailed analyses on the experiments, we discuss multiple promising directions for future research.
    % We found that the performance of existing methods declines significantly on \datasetwb, indicating that it is a challenging dataset. We also observe a positive correlation between transfer performance and domain similarity in the single-source cross-domain setting. Additionally, we investigate negative transfer in the multi-source cross-domain setting and observe that most of it comes from dissimilar source-target pairs, which suggests that domain similarity can be a useful guideline for future multi-source cross-domain research. 

\end{abstract}

==> chapters_0115/1_intro.tex <==

\section{Introduction}
\label{sec:intro}

Aspect sentiment triplet extraction \citep[ASTE;][]{peng2020knowing}, a fine-grained task in sentiment analysis \citep{hussein2018survey}, has attracted considerable interest recently \citep{peng2020knowing, xu-etal-2020-position}.  The objective of this task is to extract the sentiment triplet, comprising of an aspect term, an opinion term, and a sentiment polarity, from a given review. As depicted in Figure \ref{fig:intro-example}, an example of the sentiment triplet is ({\textit{"curly cord"}, \textit{"hate"}, \textit{NEG}}), representing a \textit{negative} sentiment toward the aspect term \textit{"curly cord"} using the opinion term {\textit{"hate"}}.

\begin{figure}[htbp] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering
\includegraphics[width=0.45\textwidth]{figures/intro-example.pdf} 
\caption{An example of the ASTE task. The terms highlighted in blue are aspect terms. The terms in orange are opinion terms. The words in green are sentiment polarities. "NULL" denotes the implicit aspect.} 
\label{fig:intro-example} %用于文内引用的标签
\end{figure}

Prior ASTE methods \citep{yan-etal-2021-unified, xu-etal-2021-learning} have achieved promising results on existing academic datasets \citep{peng2020knowing, xu-etal-2020-position, wu-etal-2020-grid}, greatly promoting the development and application of ASTE. However, these works mainly devote to designing advanced ASTE methods, the datasets they used for academic research are still relatively simple and there are still gaps between these datasets and real-world scenarios, in terms of length, expression diversity, domain distribution, etc. For instance, most reviews in existing datasets are of short length, with an average of 16 words per review, while reviews in real-world scenarios are longer (an average of more than 50 words). Additionally,  expressions used in these datasets are typically simple and straightforward, with limited diversity in lexicality and syntactic. Furthermore, existing datasets typically contain two domains, i.e., restaurant and laptop, with very limited domain distributions. In a nutshell, these gaps hide the complexity of real-world scenarios, and therefore, impede the exploration to fully understand and address the challenges presented in real-world ASTE tasks.

% while reviews in real-world scenarios are longer (average of more than 50 words)
% In contrast, real-world reviews are more complex and various in length, expression diversity, domain shift, etc. 

%Prior ASTE methods \citep{yan-etal-2021-unified, xu-etal-2021-learning} have achieved promising results on existing datasets \citep{peng2020knowing, xu-etal-2020-position, wu-etal-2020-grid}. Based on existing datasets \citep{peng2020knowing, xu-etal-2020-position, wu-etal-2020-grid}, researchers have carried out extensive research on the ASTE task, promoting the development and application of ASTE. However,  real-world scenarios tend to be complex and existing datasets are limited to represent real-world scenarios. For instance, most reviews in existing datasets are of short length, with an average of 16 words per review. Additionally, the expression used in these reviews is typically simple and straightforward, with limited diversity in terms of idiomatic phrases and colloquialisms. Furthermore, existing datasets are typically limited to only two domains, usually restaurants and laptops. These limitations in the datasets restrict the ability to accurately depict the complexity of real-world scenarios, and therefore, impede the ability to fully understand and address the challenges presented in real-world ASTE tasks.


\input{figures/fig-data-cmp.tex}
\input{tables/data_comparison_new.tex}

In order to bridge the gap and better simulate real-world scenarios, we  create a new dataset, named Diversified Multi-domain ASTE (\datasetwb), which is manually annotated to provide a more diverse and realistic set of reviews for the task. As Table~\ref{tab:cmp} and Figure~\ref{fig:intro-cmp} shows, the key characteristics of \dataset can be summarized as follows: (1) \textbf{Various lengths}: \dataset covers reviews of various lengths, ranging from 1 to 250 words, with an average of 59 words per review. (2) \textbf{Diverse expressions}: more POS and dependency n-grams show a wide variety of lexical bundles and syntactic in \datasetwb, 
%the reviews of \dataset use a wide variety of idiomatic phrases, colloquialisms, and figurative language, 
which can better represent the complexity and diversity of real-world scenarios. (3) \textbf{More aspect types}: \dataset  includes triplets annotated with both implicit and explicit aspect terms, providing  a more comprehensive understanding of the target being discussed. (4) \textbf{More domains}: \dataset covers eight domains, enabling more comprehensive research in ASTE like single-source and multi-source domain adaptation.
To summarize, these characteristics make \dataset a better benchmark to verify the ability of ASTE approaches in real-world scenarios.
% To summarize, these characteristics allow the model to better handle the variability present in the data encountered in actual usage.
 
To thoroughly investigate the challenges introduced by \dataset and explore promising directions for future ASTE research, we implement several representative methods and empirically evaluate \dataset under multiple settings:
\begin{itemize}
    \item In-domain results show that the performance of current models declines significantly on \datasetwb. And analysis reveals that \textit{long reviews, complex sentences, and implicit aspect terms make \dataset a challenging dataset}.
    \item In the single-source domain adaptation setting, we 
    %analyse the factors that impact transfer performance and 
    observe a positive correlation between transfer performance and domain similarity. But simply learning domain-invariant features may lead to the loss of task-specific knowledge, which suggests that \textit{reducing domain discrepancy while keeping the task-specific knowledge can be a future direction}.
    \item We observe the \textit{negative transfer} \citep{Rosenstein2005} in the multi-source domain adaptation setting, 
    % we investigate the phenomenon of negative transfer in the multi-source cross-domain setting 
    and find the negative transfer occurs mainly in dissimilar source-target pairs. This indicates that \textit{the domain similarity may be a useful guideline for domain selection} in future multi-source cross-domain ASTE research.
\end{itemize}
  Overall, the results of \dataset on multiple settings provide a deeper understanding of the challenges and future directions for ASTE research. We believe this work will bring a valuable research resource and benchmark for the community.

% The main contributions of this paper can be summarized as follows: 
% \begin{itemize}
%     \item We present a new dataset, \datasetwb, which is manually annotated to provide more diverse and realistic reviews for the ASTE task.
%     \item We carry out extensive experiments in multiple scenarios and provide promising directions for future research.
%     \item \XT{what can we provide to the community?}
% \end{itemize}






==> chapters_0115/3_dataset.tex <==
\input{tables/data_statistics.tex}
% \input{tables/data_comparison.tex}


\section{Dataset}
\label{sec:dataset}

% To better investigate the cross-domain ASTE task, we construct a Multi-domain ASTE dataset (\datasetwb). 
To construct a dataset that is more representative of real-world scenarios, we manually annotate a new dataset, named Diversified Multi-domain ASTE (\datasetwb).  In this section, we first present a detailed description of the data collection and annotation process. Then we demonstrate the superiority of \datasetwb, through a comparison with previous datasets in terms of key statistics and characteristics.

\subsection{Collection}
The data collection process of \dataset is carried out in three stages:
(1) We select the Amazon dataset \citep{ni-etal-2019-justifying} as our source of data due to its large volume of reviews from various regions around the world, which aligns with the goal of creating a dataset that is more representative of real-world scenarios.
(2) We select four of the most popular domains from the Amazon dataset (Appendix \ref{sec:app-dataset}), and randomly sample a portion of the data for annotation.
(3) To further enable comprehensive exploration of ASTE like domain adaptation settings, we additionally sample four additional domains and annotate a smaller portion of the data for testing in domain adaptation settings.

\subsection{Annotation}
\label{sec:annotation}

\paragraph{Simplified Annotation Guidelines \footnote{Due to the space limitation, we present detailed labeling guidelines in Appendix \ref{sec:app-guideline}.}.}Following \citet{peng2020knowing,xu-etal-2020-position,wu-etal-2020-grid}, we annotate \textit{(aspect term, opinion term, sentiment polarity)} triplets for each review, which may include multiple sentences.
An \textit{aspect term} refers to a part or an attribute of products or services.
Sometimes, the aspect term may not appear explicitly in the instance, i.e., implicit aspect terms \citep{poria2014rule}. We keep the triplets with implicit aspect terms.
An \textit{opinion term} is a word or phrase that expresses opinions or attitudes toward the aspect term.
A \textit{Sentiment polarity} is the sentiment type of the opinion term, which is divided into three categories: positive, negative, and neutral.
It is worth noting that one aspect term can be associated with multiple opinion terms and vice versa. 

\paragraph{Annotation Process.} 
In order to ensure the quality of the annotation, we employed 14 workers (annotators) to perform the annotation and 4 workers (verifiers) to perform 
 the quality-assurance sampling. Both groups are compensated based on the number of annotations. The annotation process is carried out using a train-trial-annotate-check procedure.
(1) \textit{Train}: All workers are trained on the task of annotation.
(2) \textit{Trial}: All workers try to annotate a small portion of the data to familiarize themselves with the task and to receive feedback on their annotations. Workers are required to reach 95\% accuracy in labeling before proceeding to the next phase.
(3) \textit{Annotate}: The annotators are responsible for annotating the data on a daily basis.
(4) \textit{Check}: The verifiers sampled 20\% of the annotations each day to ensure accuracy. If the accuracy of an annotator is found to be below 95\%, the data annotated by that worker for that day would be re-done until meet the accuracy requirement. Otherwise, the annotations are accepted.

\subsection{Statistics and Characteristics}
% The basic statistics of \dataset are shown in Table \ref{tab:statistics}. \dataset covers eight domains. According to the number of reviews in the Amazon dataset, we select Electronics, Fashion, Beauty, and Home as source domains because they are the leading fields of e-commerce, and there are massive reviews for these domains. We select Book, Pet, Toy, and Grocery as target domains because they have fewer reviews and are very different from each other. 
% For the source domains, we annotate more data and divide data into training, development, and test sets with a ratio of 7: 1: 2. For the target domains, we annotate fewer data and divide target data into development and test sets with a ratio of 1: 2 since we study the unsupervised domain adaptation setting.
% Among the eight domains, we select \XT{} Electronics, Fashion, Beauty, and 
% % 选择领域差异较大的四个作为源领域，然后选择领域差异多样化的作为目标领域。
% Home as source domains and annotate more data. Then we select Book, Pet, Toy, and Grocery as target domains and annotate fewer data. For the source domains, we divide data into training, development, and test sets with a ratio of 7: 1: 2. 
% For the target domains, we divide target data into development and test sets with a ratio of 1: 2 since we study more challenging unsupervised domain adaptation. 

To provide a deeper understanding of our proposed dataset, we present a series of statistics and characteristics in this section.

\paragraph{Various Lengths.} Figure \ref{fig:intro-length} illustrates the comparison of review length between \citet{xu-etal-2020-position} and \datasetwb. We find that \dataset contains reviews of more varied lengths. And Table \ref{tab:cmp} demonstrates that the average length of \dataset is 3.6 times that of \citet{xu-etal-2020-position}. 

\paragraph{Diverse Expressions.} We quantify the expression diversity by counting the vocabulary size, n-grams in part-of-speech (POS) sequences and dependency parsing (DP) trees \footnote{For the DP tree, we treat the parent node and child node as neighbors.}.  Figure \ref{fig:intro-pos} shows the comparison of POS 2-grams between \citet{xu-etal-2020-position} and \datasetwb. The results indicate that \dataset contains reviews with diverse expressions.  And Table \ref{tab:cmp} shows that the number of n-grams of POS and DP trees in \dataset is significantly higher than those of other datasets, with the number of 4-grams being about 3 times that of other datasets. Besides, the vocabulary size of \dataset is about 3 times that of other datasets. These statistics indicate that the reviews in \dataset are more diverse and complex.

\paragraph{More Aspect Types.} Table \ref{tab:cmp} shows that \dataset not only contains more explicit aspect terms than existing datasets but also includes annotations of implicit aspect terms, which constitute a large proportion. This provides a more comprehensive understanding of the target being discussed.
\paragraph{More Domains.} Table \ref{tab:cmp} illustrates that our dataset comprises four times the number of domains compared to existing datasets. Furthermore, the first four domains presented in Table \ref{tab:statistics}, which are characterized by a larger amount of annotated data, represent leading fields in e-commerce platforms (Appdenix \ref{sec:app-dataset}), providing a more realistic representation of popular topics. Additionally, we include an additional four domains with less annotated data to enable a more comprehensive analysis of the domain adaptation setting.


In summary, \dataset is a more realistic and diversified dataset, providing a suitable testbed to verify the ability of ASTE methods in real-world scenarios.
% providing more challenges to the ASTE task.

% In Table \ref{tab:cmp}, we further compare our dataset with existing representative datasets \citep{peng2020knowing, wu2020grid, xu2020position} in ASTE. First, we include \textbf{more domains} and instances in \datasetwb. The number of instances and domains in our dataset is about 1.3 and 4 times of previous datasets, respectively.  Second, the reviews in \dataset are \textbf{diversified}. The review length in our dataset is about 3.6 times the previous one. Besides, we investigate the expression diversity of our reviews by counting the n-grams in part-of-speech (POS) sequences and dependency parsing (DP) trees \footnote{For the DP tree, we treat the parent node and child node as neighbors.}. The comparison results show that the number of n-grams of POS and DP trees in \dataset is significantly higher than that of other datasets. And the number of 4-grams is even more than twice that of other datasets.
% Moreover, \dataset contains both \textbf{implicit and explicit aspects} while the others only annotate explicit aspects. 



==> chapters_0115/main.tex <==

\input{chapters_0115/0_abstract}
\input{chapters_0115/1_intro}
\input{chapters_0115/2_related_work}
\input{chapters_0115/3_dataset}

\input{chapters_0115/4_experiment_settings/main.tex}
\input{chapters_0115/5_results/main.tex}
\input{chapters_0115/6_conclusion}
\input{chapters_0115/7_limitations.tex}
\bibliography{anthology,custom}
\bibliographystyle{acl_natbib}

\appendix

\input{chapters_0115/8_appendix/main.tex}

==> tables/app_data_comparison.tex <==
\begin{table*}[h]
    \small
    \centering
    \newcolumntype{Z}{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}X}
    % \begin{tabularx}{\textwidth}{ZZZZZZ}
    \begin{tabular}{l c c c c c c c c c c c c }
    
    \toprule
    Dataset & \#D & \#I & \#W/\#I & \#T & \#IA & \#IO & \#T/\#I & POS \#n-gram & DP \#n-gram \\
    \midrule
    \citet{cai-etal-2021-aspect}             & 2 & 6360 & 15.46 & 9288 & 2099 & 2227 & 1.46 & 13.43/14.97/15.33 & 12.47/13.05/13.20\\
    \citet{zhang-etal-2021-aspect-sentiment} & 1 & 3704 & 14.50 & 5682 & 1277 & 0    & 1.53 & 12.69/14.18/14.55 & 11.82/12.38/12.51 \\
    Ours & 8 & 7524 & 59.68 & 28233 & 11945 & 0 & 3.75 &36.67/52.11/57.92 &  35.08/40.20/41.93 \\
    \bottomrule
    \end{tabular}
    \caption{Comparisons between \dataset and existing representative ASTE datasets. 
    %$\mathcal{D}_P, \mathcal{D}_W,$ and $\mathcal{D}_X$ indicate the dataset provided by \citet{peng2020knowing}, \citet{wu-etal-2020-grid}, and \citet{xu-etal-2020-position} respectively. 
    \#D, \#I, \#W, \#T, \#IA, and \#IO denote the numbers of domains, instances, words, triplets, triplets with implicit aspects, and triplets with implicit opinions, respectively.
    And \#n-gram denotes the numbers of 2/3/4-grams in part-of-speech sequences or dependency parsing trees per reviews.}
    \label{tab:app-cmp}
\end{table*}

==> tables/cross_4to1.tex <==
\begin{table}[t]
    \small
    \centering
    \newcolumntype{Z}{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}X}
    % \begin{tabularx}{\textwidth}{ZZZZZZ}
    \begin{tabular}{l c c c c c}
    \toprule
    Method      & Book   & Grocery   & Toy   & Pet   &AVE\\
    \midrule
    BMRC        & 35.89 & 42.21 & 45.10 & 40.11 & 40.83\\
    BART-ABSA   & 40.88 & 44.03 & 48.37 & 42.98 & 44.07\\
    GAS         & 38.40 & 44.80 & 46.28 & 41.99 & 42.87\\
    Span-ASTE   & 41.50 & 46.35 & 50.35 & 43.77 & 45.49\\
    \bottomrule
    \end{tabular}
    \caption{Comparison results of transferring from four source domains to different target domains.
    }
    \label{tab:4-1}
\end{table}

==> tables/cross_dataset.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}[0.45\textwidth]{lcccc}
%     \toprule
%           & 14Res & 15Res & 16Res & 14Lap \\
%     \midrule
%         Electronics & 39.81 & 39.58 & 45.35 & 29.62 \\
%         Beauty      & 35.97 & 36.32 & 41.23 & 26.02 \\
%         Fashion     & 39.57 & 38.80 & 45.66 & 30.05\\
%         Home        & 34.09 & 35.75 & 41.95 & 32.14\\
%     \bottomrule
%     \end{tabular}
%     \caption{Micro-F1 scores for cross-dataset on transferring from \dataset to \citet{xu-etal-2020-position}.}
%     \label{tab:my_label}
% \end{table}

% \begin{table}[]
%     \centering
%     \begin{tabular}[0.45\textwidth]{lcccc}
%     \toprule
%          & Electronics & Beauty & Fashion & Home \\
%     \midrule
%         14Lap & 14.18 & 13.90 & 12.38 & 8.83\\
%         14Res & 12.48 & 13.47 & 11.53 & 9.76\\
%         15Res & 13.32 & 14.08 & 12.32 & 9.68\\
%         16Res & 13.92 & 12.98 & 16.08 & 11.51\\
%     \bottomrule
%     \end{tabular}
%     \caption{Micro-F1 scores for cross-dataset on transferring from \citet{xu-etal-2020-position} to \datasetwb.}
%     \label{tab:my_label}
% \end{table}

\begin{table*}
\parbox{.45\linewidth}{
    \centering
    \small
\begin{tabular}[0.45\textwidth]{lcccc}
    \toprule
          & 14Res & 15Res & 16Res & 14Lap \\
    \midrule
        Electronics & 39.81 & 39.58 & 45.35 & 29.62 \\
        Beauty      & 35.97 & 36.32 & 41.23 & 26.02 \\
        Fashion     & 39.57 & 38.80 & 45.66 & 30.05\\
        Home        & 34.09 & 35.75 & 41.95 & 32.14\\
    \bottomrule
    \end{tabular}
    \caption{F1 scores on Span-ASTE of cross-dataset transfer from \dataset to \citet{xu-etal-2020-position}.}
    \label{tab:maste2xu}
}
\hfill
\parbox{.45\linewidth}{
    \centering
    \small
    \begin{tabular}[0.45\textwidth]{lcccc}
    \toprule
         & Electronics & Beauty & Fashion & Home \\
    \midrule
        14Res & 14.18 & 13.90 & 12.38 & 8.83\\
        15Res & 12.48 & 13.47 & 11.53 & 9.76\\
        16Res & 13.32 & 14.08 & 12.32 & 9.68\\
        14Lap & 13.92 & 12.98 & 16.08 & 11.51\\
    \bottomrule
    \end{tabular}
    \caption{F1 scores on Span-ASTE of cross-dataset transfer from \citet{xu-etal-2020-position} to \datasetwb.}
    \label{tab:xu2maste}
}
\end{table*}


==> tables/data_comparison.tex <==
\begin{table*}[h]
    \small
    \centering
    % \begin{tabularx}{\textwidth}{X|X|X|X|X|X}
    \newcolumntype{Z}{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}X}
    % \begin{tabularx}{\textwidth}{ZZZZZZ}
    \begin{tabular}{l l c c c c}
    
    \toprule
    \multicolumn{2}{c}{~}     &\citet{peng2020knowing}& \citet{wu-etal-2020-grid}  & \citet{xu-etal-2020-position} & \dataset \\
    \midrule
    \multicolumn{2}{c}{\#Domain}               & 2     & 2     & 2     & 8\\
    \midrule 
    \multicolumn{2}{c}{\#Instance}             & 6037  & 6009  & 5989  & 7524\\
    \midrule
    \multicolumn{2}{c}{\#Sentence}             & 11948 & 11884 & 11845  & 36871\\
    \midrule
    \multicolumn{2}{c}{\#Sentence/\#Instance}  & 1.98  & 1.98  & 1.98  & 4.90\\
    \midrule
    \multicolumn{2}{c}{\#Triplet}              & 9309  & 10390 & 10252 & 28233\\
    \midrule
    \multicolumn{2}{c}{\#Triplet/\#Instance}   & 1.54  & 1.73  & 1.71  & 3.75\\
    \midrule
    \multicolumn{2}{c}{\#IA Triplet}           & 0     & 0     & 0     & 11945\\
    \midrule 
    \multicolumn{2}{c}{\#Word/\#Instance}      & 16.49 & 16.46 & 16.43 & 59.68\\
    % \midrule 
    % \multirow{3}*{POS v0}      &\#2-gram           & 269   & 266   & 266   & 300\\
    % % \cline{2-6}
    %                         &\#3-gram           & 2316  & 2306  & 2303  & 3275\\
    % % \cline{2-6}
    %                         &\#4-gram           & 10147 & 10101 & 10073 & 20120\\
    % % \cline{2-6}
    % \midrule 
    % \multirow{3}*{DP Tree v0}  &\#2-gram           & 672   & 670   & 670   & 993\\
    % % \cline{2-6}
    %                         &\#3-gram           & 2727  & 2732  & 2725  & 5400\\
    % % \cline{2-6}
    %                         &\#4-gram           & 4635  & 4620  & 4612  & 11564\\
    \midrule 
    \multirow{4}*{POS}   &\#1-gram           & 8.38   & 8.37   & 8.36   & 11.95\\
    % \cline{2-6}
                            &\#2-gram           & 14.25  & 14.22  & 14.20  & 36.67\\
                            &\#3-gram           & 16.05  & 16.02  & 16.00  & 52.11\\
    % \cline{2-6}
                            &\#4-gram           & 16.52  & 16.48  & 16.46 & 57.92\\
    % \cline{2-6}
    \midrule 
    \multirow{3}*{DP Tree}  &\#1-gram        & 9.89   & 9.87   & 9.86   & 18.04\\
    % \cline{2-6}
                            &\#2-gram           & 13.51  & 13.48  & 13.46  & 35.08\\
                            &\#3-gram           & 14.24  & 14.21  & 14.19  & 40.20\\
    % \cline{2-6}
                            &\#4-gram           & 14.43  & 14.40  & 14.38  & 41.93\\
    \bottomrule
    \end{tabular}
    \caption{Comparisons between \dataset and existing representative ASTE datasets.  \#Domain, \#Instance, \#Sentence, \#Triplet, and \#IA Triplet denote the numbers of domains, instances, sentences, triplets, and triplets with implicit aspects, respectively.
    And \#n-gram denotes the numbers of n-grams in part-of-speech sequences or dependency parsing trees per instance.}
    \label{tab:cmp}
\end{table*}


==> tables/multi_source.tex <==
% \begin{table*}[]
%     \small
%     \centering
%     \begin{tabular}{lcccccc}
%     \toprule 
%          & B + H $\to$ K & F + H $\to$ K & B + E + H $\to$ K & E + F + H $\to$ K & B + F + H $\to$ K & A $\to$ K  \\
%     \midrule
%     Triplets & 41.31 & 42.40 & 41.21 & 41.44 & 41.73 & 41.50\\
%     Aspect   & 60.30 & 61.43 & 60.38 & 59.64 & 61.07 & 60.86\\
%     Opinion  & 49.18 & 49.53 & 49.25 & 48.60 & 49.39 & 50.15\\
%     AO-pair  & 44.21 & 45.18 & 44.15 & 44.38 & 44.70 & 44.65\\
%     \bottomrule
%     \end{tabular}
%     \caption{Comparison results of multi-source cross-domain ASTE on Span-ASTE. We present part of the results with the book as the target domain. We use abbreviations due to space limitation: B: Beauty, H: Home, F: Fashion, E: electronics, K: Book. This table shows the phenomenon of negative transfer, e.g., B + H $\to$ K > B + E + H $\to$ K.\XT{}}
%     % XT: 要不要改成在Span-ASTE上迁移到各个目标领域的，这样就可以避免triplets的问题，同时展示更多的目标领域
%     \label{tab:multi-source}
% \end{table*}


\begin{table}
    \small
    \centering
    \begin{tabular}{lcccc}
    \toprule 
    Domain    & Book & Grocery & Toy & Pet  \\
    \midrule
    B + H & 41.31 & 44.31 & 47.10 & 41.67\\
    F + H & 42.40 & 45.97 & 49.11 & 43.12\\
    B + E + H & \underline{41.21} & 45.39 & 49.33 & 43.48 \\
    E + F + H & \underline{41.44} & \underline{45.39} & 50.24 & 43.59\\
    B + F + H & \underline{41.73} & \underline{45.40} & \underline{48.55} & 43.46\\
    ALL & \underline{41.83} & 46.07 & \underline{50.16} & 45.42\\
    \bottomrule
    \end{tabular}
    \caption{Comparison results of multi-source cross-domain ASTE on Span-ASTE. We use abbreviations due to space limitation: B: Beauty, H: Home, F: Fashion, E: electronics, ALL: all the source domains. We underline the situations of negative transfer.}
    % XT: 要不要改成在Span-ASTE上迁移到各个目标领域的，这样就可以避免triplets的问题，同时展示更多的目标领域
    \label{tab:multi-source}
\end{table}

==> tmp.tex <==
\begin{abstract}
This document is a supplement to the general instructions for *ACL authors. It contains instructions for using the \LaTeX{} style files for ACL conferences. 
The document itself conforms to its own specifications, and is therefore an example of what your manuscript should look like.
These instructions should be used both for papers submitted for review and for final versions of accepted papers.
\end{abstract}

\section{Introduction}

These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.
\bibliography{anthology,custom}
\bibliographystyle{acl_natbib}

\appendix

\section{Example Appendix}
\label{sec:appendix}

This is an appendix.
